Fixed-Point Approaches to Computing Bertrand-Nash Equilibrium Prices Under Mixed Logit Demand: A Technical Framework for Analysis and Efficient Computational Methods

This article presents a detailed technical framework for modeling with Bertrand-Nash equilibrium prices under Mixed Logit demand. Two coercive fixed-point equations provide more stable computational methods than those obtained from the literal first-order conditions. Assumptions to justify derivation and use of these equations are provided. A brief discussion of a GMRES-Newton method with hookstep globalization strategy originally due to Viswanath is also given. This article can be considered a supplement to an article by the authors forthcoming in the journal {\em Operations Research}.

==> FULLframework.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SECTION X : MIXED LOGIT  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
\section{Fixed-Point Equations for Equilibrium Prices Under Mixed Logit Models}
\label{ECSEC:MixedLogit}
	
	In this section we derive two fixed-point equations for (local) equilibrium prices under Mixed Logit models. Such models are very popular in empirical applications and dense in the class of Random Utility Models (RUM) \citep{McFadden00}. Our description of the Mixed Logit model in Section \ref{SUBSEC:PPCP} follows \cite[Chapter 5]{Train03} and is more general than the description now standard in many empirical papers. This generality is required to capture a variety of models currently used in practice, while being broad enough to admit examples that have perhaps not yet appeared. The material in Sections \ref{SUBSEC:FirmsCostsProfits}-\ref{SUBSEC:EquilibriumAndTheSSCs} closely follows the discussions in \cite{Nevo00b} and \cite{Dube02}, among others. In the E-Companion, Section \ref{ECSEC:Framework}, we provide a detailed derivation of the framework for an arbitrary RUM. Sections \ref{SUBSEC:ChoiceProbabilityDerivatives}-\ref{SUBSEC:ZetaMap} focus on material not prominent in the existing literature. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{Consumers, Products, and Choice Probabilities}
	\label{SUBSEC:PPCP}
	
	A collection of firms offer a total of $J \in \N$ products to a population of individuals (or households). Each product $j \in \N(J)$ is endowed with a price, $p_j \in \set{P} = [0,\infty)$, and a vector of $K \in \N$ product ``characteristics'' $\vec{x}_j \in \set{X} \subset \R^K$. These characteristics allow products to be differentiated in ways not captured by price alone. Individuals are also identified by a vector of characteristics, or ``demographics,'' from some set $\set{T}$. An individual characterized by $\bsym{\theta} \in \set{T}$ receives the (random) utility $U_j(\bsym{\theta},\vec{x}_j, p_j) = u(\bsym{\theta},\vec{x}_j, p_j) + \set{E}_j$ from purchasing product $j \in \N(J)$, and $U_0(\bsym{\theta}) = \vartheta(\bsym{\theta}) + \set{E}_0$ for forgoing purchase of any of these products or ``purchasing the outside good.'' Here $u : \set{T} \times \set{X} \times \set{P} \to [-\infty,\infty)$ is a product-specific systematic utility function, $\vartheta : \set{T} \to \R$ is a valuation of the no-purchase option or ``outside good,'' and $\bsym{\set{E}} = \{ \set{E}_j \}_{j = 0}^J$ is a random vector of i.i.d. standard extreme value variables. Several examples of $u$ and $\vartheta$ are given below. 
	
	The individual characteristics $\bsym{\theta}$ can include both observed and ``unobserved'' demographic variables. Observed demographics are measurable characteristics such as income, age, or number of children that have a systematic influence on the value of different bundles of product characteristics and price. Unobserved demographics, also often called ``random coefficients'' \citep{Nevo00b,Train03}, characterize individual-specific heterogeneity that is assumed to exist, but is not systematically modeled. In this article, we suppose only the existence of $\set{T}$ and a probability distribution $\mu$ over $\set{T}$. Several examples are given below. 
	
	Demand for each product $j$ is characterized by choice probabilities $P_j : \set{P}^J \to [0,1]$ derived from (random) utility maximization. As is well known the choice probabilities for an individual characterized by $\bsym{\theta} \in \set{T}$ are those of the Logit model \citep[Chapter 3]{Train03}:
	\begin{equation*}
		P_j^L(\bsym{\theta},\vec{p})
			= \frac{ e^{u_j(\bsym{\theta},p_j)} }
				{ e^{\vartheta(\bsym{\theta})} + \sum_{k=1}^J e^{u_k(\bsym{\theta},p_k)} }
	\end{equation*}
	where $e^{-\infty} = 0$, $\vec{p} \in \set{P}^J$ denotes the vector of all product prices, and we suppress the dependency of utility on product characteristics by admitting product-specific utility functions $u_j : \set{T} \times \set{P} \to [-\infty,\infty)$ for all $j$, defined by $u_j(\bsym{\theta},p) = u(\bsym{\theta},\vec{x}_j,p)$ for all $(\bsym{\theta},p) \in \set{T} \times \set{P}$. The Mixed Logit choice probabilities $P_j(\vec{p})$ follow from integrating over the distribution of individual characteristics: $P_j(\vec{p}) = \int P_j^L(\bsym{\theta},\vec{p}) d\mu(\bsym{\theta})$; See \cite{Train03}. This ``mixing'' of a family of Logit choice probabilities provides the Mixed Logit class of choice models its name. 
	
	A Mixed Logit model is truly specified by choosing $\set{T}$, $\mu$, $u$, and $\vartheta$. Before continuing with our general framework, we review several examples:
	
	\begin{example} \citep{Boyd80}
		\label{BoydExample}
		Take $\set{T} = \set{P} \times \R^K$, denoting $\bsym{\theta} = (\alpha,\bsym{\beta})$ for $\alpha \in \set{P}$ and $\bsym{\beta} \in \R^K$, and set $u(\alpha,\bsym{\beta},\vec{x},p) = - \alpha p + \bsym{\beta}^\top\vec{x}$. $\vartheta(\alpha,\bsym{\beta}) = -\infty$ for all $(\alpha,\bsym{\beta})$. $\alpha$ and $\bsym{\beta}$ are lognormally distributed over the population. \Halmos
	\end{example}
	
	\begin{example} \citep{Berry95}
		\label{BLPExample}
		Take $\set{T} = \set{P} \times \R^K \times \R$, denoting $\bsym{\theta} = (\phi,\bsym{\beta},\beta_0)$ for $\phi \in \set{P}$, $\bsym{\beta} \in \R^K$, and $\beta_0 \in \R$. Set 
		\begin{equation*}
			u(\phi,\bsym{\beta},\vec{x},p) 
				= \left\{ \begin{aligned}
					&\alpha \log( \phi - p ) + \bsym{\beta}^\top\vec{x} 
						&&\quad\text{if } p < \phi \\
					&-\infty &&\quad\text{otherwise}
				\end{aligned} \right .
		\end{equation*}
		and 
		\begin{equation*}
			\vartheta(\phi,\beta_0)
				= \alpha \log \phi + \beta_0
		\end{equation*}
		for some fixed coefficient $\alpha > 0$. In \cite{Berry95}, $\phi$ represents income, and is given a lognormal distribution. Generally speaking, $\phi$ represents an individual-specific {\em reservation price}; that is, a price level beyond which a given individual will never consider a product, {\em regardless} of its bundle of product characteristics. The coefficients $\bsym{\beta},\beta_0$ are independently normally distributed. \Halmos
		
%		\citeauthor{Berry95} decompose the coefficients $\bsym{\beta}$ over $N \in \N$ unobserved demographic variables with distribution $\mu^u$, respectively, as follows: $\bsym{\beta} = \bsym{\beta}^c + \bsym{\Sigma}\bsym{\set{V}}$ where $\bsym{\beta}^c \in \R^K$ are constants, $\bsym{\Sigma} \in \R^{ K \times N }$ is a diagonal coefficient matrix, and $\bsym{\set{V}}$ is a $R^N$-valued random vector with the distribution $\mu^u$.  
		
	\end{example}
	
	\begin{example} \citep{Nevo00b}
		Take $\set{T} = \set{P} \times \R^D \times \R^{(K+2)}$, denoting $\bsym{\theta} = (\phi,\vec{d},\bsym{\nu})$ for $\phi \in \set{P}$, $\vec{d} \in \R^D$, and $\bsym{\nu} \in \R^{(K+2)}$. Again, $\phi$ represents income; $\vec{d} \in \R^D$ represents a vector of $D$ observed demographic variables (which may itself include income); $\bsym{\nu} \in \R^{(K+2)}$ represents a vector of $K+2$ unobserved demographic variables: one for each product characteristic, one for price, and one for the outside good. Set 
		\begin{equation*}
			u(\phi,\vec{d},\bsym{\nu},\vec{x},p) 
				= ( \alpha + \bsym{\pi}_p^\top\vec{d} + \bsym{\sigma}_p^\top \bsym{\nu} ) ( \phi - p ) 
					+ \left( \bsym{\beta} + \bsym{\Pi}\vec{d} + \bsym{\Sigma}\bsym{\nu} \right)^\top\vec{x} 
%				= \left( \begin{bmatrix} \alpha \\ \bsym{\beta} \end{bmatrix}
%					+ \bsym{\Pi}\vec{d} + \bsym{\Sigma}\bsym{\nu} \right)^\top
%						\begin{bmatrix} \phi - p \\ \vec{x} \end{bmatrix}
		\end{equation*}
		and
		\begin{equation*}
			\vartheta(\phi,\vec{d},\bsym{\nu})
				= ( \alpha + \bsym{\pi}_p^\top\vec{d} + \bsym{\sigma}_p^\top \bsym{\nu} ) \phi 
						+ \bsym{\pi}_0^\top\vec{d} + \bsym{\sigma}_0^\top\bsym{\nu}
		\end{equation*}
		where $\alpha \in \R$, $\bsym{\beta} \in \R^K$, $\bsym{\pi}_p,\bsym{\pi}_0 \in \R^{D}$, $\bsym{\Pi} \in \R^{K \times D}$, $\bsym{\sigma}_p,\bsym{\sigma}_0 \in \R^{K+2}$, and $\bsym{\Sigma} \in \R^{K \times (K+2)}$ are coefficients. The distribution of $\vec{d}$ is estimated from available data (e.g., Census data) and $\bsym{\nu}$ is assumed to be {\em standard} independent multivariate normal. Note that this choice implies that there are individuals that prefer higher product prices, in that the coefficient on price can be positive. \cite{Berry04a} adopt a similar specification that does not have this problem by taking the coefficient on $(\phi - p)$ to be of the form $e^{( \alpha + \bsym{\pi}_p^\top\vec{d} + \bsym{\sigma}_p^\top \bsym{\nu} )}$. \Halmos
		
%		Take $\set{T} = \set{P} \times \set{P} \times \R^K$, denoting $\bsym{\theta} = (\alpha,\phi,\bsym{\beta})$ for $\alpha,\phi \in \set{P}$ and $\bsym{\beta} \in \R^K$, and set 
%		\begin{equation*}
%			u(\alpha,\phi,\bsym{\beta},\vec{x},p) 
%				= \alpha ( \phi - p ) + \bsym{\beta}^\top\vec{x} 
%		\end{equation*}
%		Again, $\phi$ represents income. \citeauthor{Nevo00b} decomposes the coefficients $\alpha,\bsym{\beta}$ over $D \in \N$ observed and $N \in \N$ unobserved demographic variables with distributions $\mu^o$ and $\mu^u$, respectively, as follows: 
%		\begin{equation*}
%			\begin{pmatrix} \alpha \\ \bsym{\beta} \end{pmatrix}
%				= \begin{pmatrix} \alpha^c \\ \bsym{\beta}^c \end{pmatrix}
%					+ \bsym{\Pi}\vec{D} + \bsym{\Sigma}\bsym{\set{V}}
%		\end{equation*}
%		where $\alpha^c \in \R$ and $\bsym{\beta}^c \in \R^K$ are constants, $\bsym{\Pi} \in \R^{(K+1) \times D}$ and $\bsym{\Sigma} \in \R^{(K+1)\times N}$ are coefficient matrices, $\vec{D}$ is a $\R^D$-valued random vector with the distribution $\mu^o$, and $\bsym{\set{V}}$ is a $R^N$-valued random vector with the distribution $\mu^u$. 
%		
%		The outside good utility is given by
%		\begin{equation*}
%			\vartheta(\phi,\beta_0)
%				= \alpha \phi + \beta_0
%			\quad\quad\text{where}\quad\quad
%			\beta_0 = \bsym{\pi}_0^\top\vec{D} + \sigma_0 \set{V}_0. \Halmos
%		\end{equation*}
		
	\end{example}
	
	\begin{example} \cite{Petrin02} modifies the models from \cite{Berry95} and \cite{Nevo00b}, taking
		\begin{equation*}
			u(\phi,\vec{d},\bsym{\nu},\vec{x},p) 
				= \alpha(\phi) \log( \phi - p )
					+ \bsym{\beta}(\phi,\vec{d},\bsym{\nu})^\top\vec{x}
		\end{equation*}
		where $\alpha : \set{P} \to \set{P}$ is a step function and $\bsym{\beta} : \set{P} \times \R^D \times \R^{K+2} \to \R^K$ is nonlinear in $(\phi,\vec{d},\bsym{\nu})$. The distribution of $\vec{d}$ is determined from the Consumer Expenditure Survey and $\bsym{\nu}$ is taken to be independent $\chi^2$ truncated at 95\%. \Halmos
	\end{example}
	
%	\begin{example} \citep{Brownstone99}
%		Take $u = p/\log \varsigma + \bsym{\beta}^\top\vec{x}$
%	\end{example}
	
%	Demand for each product $j$ is characterized by choice probabilities $P_j : \set{P}^J \to [0,1]$ derived from (random) utility maximization. As is well known the choice probabilities for an individual characterized by $\bsym{\theta} \in \set{T}$ are those of the Logit model \citep[Chapter 3]{Train03}:
%	\begin{equation*}
%		P_j^L(\bsym{\theta},\vec{p})
%%			= \Prob ( C(\vec{p}) = j \mid \bsym{\Theta} = \bsym{\theta} )
%			= \frac{ e^{u_j(\bsym{\theta},p_j)} }{ e^{\vartheta(\bsym{\theta})} + \sum_{k=1}^J e^{u_k(\bsym{\theta},p_k)} }
%%			= \left\{ \begin{aligned}
%%				&\frac{ e^{u_j(\bsym{\theta},p_j)} }{ e^{\vartheta(\bsym{\theta})} + \sum_{k=1}^J e^{u_k(\bsym{\theta},p_k)} }
%%					&&\quad\text{if } p_k < \varsigma(\bsym{\theta}) \\
%%				&\quad\quad\quad\quad 0
%%					&&\quad\text{if } p_k \geq \varsigma(\bsym{\theta}) \\
%%			\end{aligned} \right .
%	\end{equation*}
%	where $e^{-\infty} = 0$, $\vec{p} \in \set{P}^J$ denotes the vector of all product prices, and we suppress the dependency of utility on product characteristics by admitting product-specific utility functions $u_j : \set{T} \times \set{P} \to [-\infty,\infty)$ for all $j$, defined by $u_j(\bsym{\theta},p) = u(\bsym{\theta},\vec{x}_j,p)$ for all $(\bsym{\theta},p) \in \set{T} \times \set{P}$. The Mixed Logit choice probabilities $P_j(\vec{p})$ follow from integrating over the distribution of individual characteristics; see \cite{Train03}. This ``mixing'' of a family of Logit choice probabilities provides the Mixed Logit class of RUMs its name. 
	
%	We let $\vec{P} : \set{P}^J \to \triangle(J)$ denote the vector of Mixed Logit choice probabilities for all products. $\vec{P}$ need not sum to one, if the outside good is purchased with positive probability. % $P_0 = 1 - \sum_{j=1}^J P_j$ is the probability no product is chosen, or the probability of purchasing the outside good. 
	
	
	
%	Split $\bsym{\theta} = (\bsym{\psi},\bsym{\phi})$ where $\bsym{\psi}$ are observed demographics and $\bsym{\phi}$ are unobserved. When a Mixed Logit model is constructed, there are typically a known set of observed demographics $\{ \bsym{\psi}_i \}_{i=1}^I$. However in applying this model to the general population, we have to draw $\bsym{\psi}$ from an estimated distribution of observed demographic variables in the population. 
	
%	Purchases are made by a population of consumers differentiated by ``type'' variables or ``demographics'' $\bsym{\theta}$ drawn from some set $\set{T}$. These demographics may be both observed and ``unobserved'' \cite{Berry95}. Observed demographics are quantifiable characteristics such as income, age, or number of children that can have a systematic influence on the value of different combinations of product characteristics and price. Unobserved demographics, also often called ``random coefficients'' \citep{Nevo00b,Train03}, characterize individual-specific heterogeneity that is assumed to exist, but not systematically modeled. We view demographics as a random vector $\bsym{\Theta}$ with $\Prob( \bsym{\Theta} \in \set{A} ) = \int_{\set{A}} d\mu(\bsym{\theta})$, $\set{A} \subset \set{T}$, for some probability distribution $\mu$. 
	
	We now present our generalization of the systematic utility functions used in the examples above. This specification is closely related to the one introduced by \cite{Caplin91}. \cite{Morrow08a} use a similar specification to analyze equilibrium prices in simple Logit models. 
	\begin{assumption}
		\label{MixedLogitUtilityAssump}
		For all $j$, there exist functions $w_j : \set{T} \times \set{P} \to [-\infty,\infty)$ and $v_j : \set{T} \to (-\infty,\infty)$ such that the systematic utility function $u_j : \set{T} \times \set{P} \to [-\infty,\infty)$ can be written $u_j(\bsym{\theta},p) = w_j(\bsym{\theta},p) + v_j(\bsym{\theta})$. Furthermore there exists $\varsigma : \set{T} \to (0,\infty]$ such that $w_j : \set{T} \times [0,\infty] \to [-\infty,\infty)$ satisfies, for all $j$ and $\mu$-almost every (a.e.) $\bsym{\theta} \in \set{T}$, 
		\begin{itemize}
			\item[(a)] $w_j(\bsym{\theta},\cdot) : (0,\varsigma(\bsym{\theta})) \to [-\infty,\infty)$ is continuously differentiable, strictly decreasing, and finite
			\item[(b)] $w_j(\bsym{\theta},p) = -\infty$ for all $p \geq \varsigma(\bsym{\theta})$, and 
			\item[(c)] $w_j(\bsym{\theta},p) \downarrow -\infty$ as $p \uparrow \varsigma(\bsym{\theta})$. 
		\end{itemize}
		$v_j : \set{T} \to (-\infty,\infty)$ is arbitrary. 
%		\begin{itemize}
%			\item[(a)] $w_j(\bsym{\theta},\cdot) : (0,\varsigma(\bsym{\theta})) \to (-\infty,\infty)$ is continuously differentiable 
%			\item[(b)] $w_j(\bsym{\theta},\cdot) : (0,\varsigma(\bsym{\theta})) \to (-\infty,\infty)$ is  strictly decreasing
%			\item[(c)] $w_j(\bsym{\theta},p) > -\infty$ for all $p < \varsigma(\bsym{\theta})$, $w_j(\bsym{\theta},p) = -\infty$ for all $p \geq \varsigma(\bsym{\theta})$, and $w_j(\bsym{\theta},p) \downarrow -\infty$ as $p \uparrow \varsigma(\bsym{\theta})$. 
%		\end{itemize}
%		$v_j : \set{T} \to (-\infty,\infty)$ is arbitrary. 
	\end{assumption}
	
	Note that we have not restricted $\mu$, the distribution of individual characteristics, with Assumption \ref{MixedLogitUtilityAssump}. Important examples of $\mu$ from the econometrics and marketing literature include finitely supported distributions (often empirical frequency distributions for integral observed demographic variables), standard continuous distributions (e.g. normal, lognormal and $\chi^2$), truncated standard continuous distributions, finite mixtures of standard continuous distributions, and independent products of any of these types of distributions. This generality allows us to address a wide variety of otherwise disparate examples with a single notation. In particular, this generality allows us to use a single framework to treat both ``full'' Mixed Logit models defined by some $\mu$ with uncountable support and simulation-based approximations to such models. % One can view the individual characteristics as $\set{T}$-valued random vector $\bsym{\Theta}$ with the distribution $\mu$; that is, $\Prob( \bsym{\Theta} \in \set{A} ) = \int_{\set{A}} d\mu(\bsym{\theta})$, $\set{A} \subset \set{T}$. 
	
%	Some existing empirical specifications violate Assumption \ref{MixedLogitUtilityAssump} by admiting positive price coefficients for $\bsym{\theta} \in \set{T}^\prime \subset \set{T}$, where $\set{T}^\prime \subset \set{T}$ has nonzero $\mu$-measure. See, for example, \cite{Brownstone00}. This implies that $w(\bsym{\theta},\cdot)$ is increasing on $\set{T}^\prime$. If $w(\bsym{\theta},\cdot)$ is {\em not} decreasing for $\mu$-a.e. $\bsym{\theta}$, or at least {\em eventually} decreasing for $\mu$-a.e. $\bsym{\theta}$ in the sense that there are always prices large enough to ensure that $w(\bsym{\theta},\cdot)$ is decreasing for $\mu$-a.e. $\bsym{\theta}$, then profit-optimal pricing is not a well-posed problem and finite equilibrium prices will not exist. 
	
	The variable $\Sigma = \varsigma(\bsym{\theta})$ represents an individual-specific reservation price. As in the \cite{Berry95} model of Example \ref{BLPExample}, this reservation price is most often derived from household or individual income. Correspondingly, $\Sigma$ is often given a lognormal distribution to (roughly) fit empirical income data. In principle, this reservation price could be related to purchasing power derived from observed demographic variables other than income, or unobserved demographic variables such as family wealth. Conditions (b) and (c) in Assumption \ref{MixedLogitUtilityAssump} imply that the probability an individual characterized by $\bsym{\theta}$ will purchase a product is zero for any price above $\varsigma(\bsym{\theta})$ {\em and} vanishes as the price approaches $\varsigma(\bsym{\theta})$. We set $\varsigma_* = \esssup_\mu \varsigma$ and allow, but do not require, $\varsigma_* = \infty$. For example, simulation-based approximations to the \citeauthor{Berry95} demand model has $\varsigma_* < \infty$, as can be easily checked. 
	
	Note also that Condition (c) in Assumption \ref{MixedLogitUtilityAssump} ensures the continuity of $P_j^L(\bsym{\theta},\vec{p})$ at any vector of prices with some component equal to $\varsigma(\bsym{\theta})$. We must require this of the {\em Logit} choice probabilities to obtain {\em Mixed Logit} choice probabilities that are continuous on $(\vec{0},\varsigma_*\vec{1})$ for the important class of models with finitely supported $\mu$. This class includes those models derived from simulation-based approximation to ``full'' Mixed Logit models. Continuous Logit choice probabilities also imply continuous Mixed Logit choice probabilities, by the Dominated Convergence Theorem. 
	
%	Suppose instead that $\lim_{ p \uparrow \varsigma(\bsym{\theta}) } w_j(\bsym{\theta},p) > - \infty$. Let $\set{T} = \{\bsym{\theta}_t\}_{t=1}^T$ for some $T \in \N$, and take $\mu(\bsym{\theta}_t) = m_t$ where $\{ m_t \}_{t=1}^T \subset [0,1]$, $\sum_{t=1}^T m_t = 1$. Then
%	\begin{equation*}
%		P_j(\vec{p}) = \sum_{ \{ t : p_j \leq \varsigma(\bsym{\theta}_t) \} } m_t P_j^L(\bsym{\theta}_t,\vec{p})
%	\end{equation*} 
%	Order $\set{T} = \{\bsym{\theta}_t\}_{t=1}^T$ so that $\varsigma(\bsym{\theta}_t) < \varsigma(\bsym{\theta}_{t+1})$. Define $\set{A}_0 = [0,\varsigma(\bsym{\theta}_1)]$, $\set{A}_t = [\varsigma(\bsym{\theta}_t),\varsigma(\bsym{\theta}_{t+1})]$ for all $t < T$, and $\set{A}_T = [\varsigma(\bsym{\theta}_T),\infty)$, and $\set{B}_{\vec{t}} = \set{A}_{t_1} \times \dotsc \times \set{A}_{t_J}$ for any $\vec{t} \in \{0,\dotsc,T\}^J$. $P_j$ is continuous only in the interior of each $\set{B}$. 
%	
%	For example, the restricted choice probability function $P_j(\cdot,\vec{p}_{-j}) : \set{P} \to [0,1]$ is discontinuous at the $T$ points $\varsigma(\bsym{\theta}_i)$. Fix $\tau \in \{2,\dotsc,T-1\}$ and $h > 0$ be small enough so that
%	\begin{equation*}
%		\varsigma(\bsym{\theta}_{\tau-1}) 
%			< \varsigma(\bsym{\theta}_\tau) - h 
%			< \varsigma(\bsym{\theta}_\tau) 
%			< \varsigma(\bsym{\theta}_\tau) + h 
%			< \varsigma(\bsym{\theta}_{\tau+1}). 
%	\end{equation*} 
%	For any such $h$, 
%	\begin{equation*}
%		P_j(\varsigma(\bsym{\theta}_\tau) - h,\vec{p}_{-j}) 
%			= \sum_{t \leq \tau} m_t P_j^L(\bsym{\theta}_t,\varsigma(\bsym{\theta}_\tau) - h,\vec{p}_{-j}) 
%	\end{equation*} 
%	and
%	\begin{equation*}
%		P_j(\varsigma(\bsym{\theta}_\tau) + h,\vec{p}_{-j}) 
%			= \sum_{t < \tau} m_t P_j^L(\bsym{\theta}_t,\varsigma(\bsym{\theta}_\tau) + h,\vec{p}_{-j}). 
%	\end{equation*}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{Firms, Costs, and Profits}
	\label{SUBSEC:FirmsCostsProfits}
	
	There are $F \in \N$ firms, each of which offers some subset $\set{J}_f \subset \N(J)$ of the $J$ products offered to the consumer population. In Bertrand competition, each firm $f$ chooses the prices of the products indexed by $j \in \set{J}_f$ prior to some purchasing period in which consumers opt to purchase one, or none, of the products offered by all firms. All prices remain fixed during this purchasing period, and firms commit to satisfying any demand that may arise \citep{Baye08}. 
	
	Firms choose these prices to maximize their expected profits, equivalent to maximizing
	\begin{equation}
		\label{ExpectedProfits}
		\hat{\pi}_f(\vec{p}_f,\vec{p}_{-f}) 
			= \vec{P}_f(\vec{p})^\top ( \vec{p}_f - \vec{c}_f )
			= \sum_{j \in \set{J}_f} P_j(\vec{p}) ( p_j - c_j )
	\end{equation}
	where $\vec{p}_f \in \set{P}^{J_f}$ denotes the vector of prices for products offered by firm $f$, $\vec{p}_{-f}$ denotes the prices of products offered by competing firms, $\vec{c}_f \in \set{P}^{J_f}$ denotes the vector of {\em fixed} unit costs incurred by firm $f$ in offering these products, and $\vec{P}_f(\vec{p})$ denotes the vector of choice probabilities for firm $f$'s products as a function of all prices. 
	
%	Negative subscripts denote competitor's variables as in, for instance, $\vec{p}_{-f} \in \R^{J_{-f}}$, where $J_{-f} = \sum_{g \neq f} J_g$, is the vector of prices for products offered by all of firm $f$'s competitors. In writing ``$f(j)$'' for some $j \in \N(J)$, we mean the unique $f \in \N(F)$ such that $j \in \set{J}_f$. 
	
	Fixed unit costs are required because of the firms' ``commitment'' to produce whatever demand arises during the purchasing period \citep{Baye08}. If unit costs may depend on production volumes, or at least expected production volumes, prices influence costs as prices influence both expected and actual production volumes. See our derivation in the E-Companion (Section \ref{ECSEC:Framework}) for more detail. Our framework is easily modified to include a dependence of costs on production volumes. This dependence is, in fact, common in the theoretical literature; see, e.g. \cite{Milgrom90, Caplin91, Mizuno03, Cabral05, Gallego06}. While the specific equations employed in this article change with quantity-dependent costs, the spirit of the methods does not change. 
	
%	\cite{Esteban07} state this another way: ``[A]n implicit assumption of the Bertrand price-setting model is flexible capacity'' \citep[pg. 334]{Esteban07}. 
%	In principle, the framework we have described can be modified to include a dependence of costs on production volumes. This is common in the theoretical literature; see, e.g. \cite{Milgrom90, Caplin91, Mizuno03, Cabral05, Gallego06}. However most empirical applications that include unit costs that vary with production volume do not include the derivative(s) of the cost function with respect to production volume in the first-order condition for equilibrium. To focus on the forms used most often in the empirical literature, we must assume unit costs are fixed. While the specific equations we employ in this article change with quantity-dependent costs, the spirit of our methods does not change. 

	We present a technical assumption that ensures that profits are not only bounded, but vanish as prices approach $\varsigma_*$. 
	
	\begin{assumption}
		\label{A1}
		For all $j$ there exists some $r_j : \set{T} \to (1,\infty)$ and some $\bar{p}_j : \set{T} \to \set{P}$ satisfying
		\begin{equation}
			\label{PCond}
			\sup \Big\{ \; p \mu(\{ \bsym{\theta} : \bar{p}(\bsym{\theta}) > p \}) \; : \; p \in (0,\varsigma_*) \; \Big\} < \infty. 
		\end{equation} 
		such that 
		\begin{equation}
			\label{UtilityBound}
			u_j(\bsym{\theta},p) \leq -r_j(\bsym{\theta}) \log p + \vartheta(\bsym{\theta})
		\end{equation}
		for all $p \geq \bar{p}_j(\bsym{\theta})$, $\mu$-a.e. 
	\end{assumption}
	Eqn. (\ref{UtilityBound}) ensures that the integrand in
	\begin{equation*}
		\hat{\pi}_f(\vec{p})
			= \int \left( \sum_{j \in \set{J}_f} P_j^L(\bsym{\theta},\vec{p})(p_j - c_j) \right) d\mu(\bsym{\theta})
	\end{equation*}
	vanishes $\mu$-a.e.; see also \cite{Morrow08a}. Eqn. (\ref{PCond}) ensures that the Dominated Convergence Theorem can be applied as $\vec{p} \to \varsigma_*\vec{1}$. 
	
	Note that if $\varsigma(\bsym{\theta}) < \infty$ then Eqn. (\ref{UtilityBound}) holds for {\em any} $r(\bsym{\theta}) > 1$ by taking $\bar{p}(\bsym{\theta}) = \varsigma(\bsym{\theta})$. Furthermore, if $\varsigma_* < \infty$, then Eqn. (\ref{PCond}) is trivial. 
	
	To further analyze this assumption, we assume $\varsigma_* = \infty$. Even in this case, both assumptions are quite weak. The utility bound Eqn. (\ref{UtilityBound}) admits any utility function that is concave in price. To further consider Eqn. (\ref{PCond}), we define $Z = \bar{p}(\bsym{\Theta})$, where $\bsym{\Theta}$ is the $\set{T}$-valued random variable with $\Prob( \bsym{\Theta} \in \set{A} ) = \mu(\set{A}) = \int_{\set{A}} d\mu(\bsym{\theta})$; if $\varsigma(\bsym{\theta}) < \infty$. for $\mu$-a.e. $\bsym{\theta}$, then we can take $Z = \Sigma$. Then Eqn. (\ref{PCond}) can be re-written $\sup\{ p \Prob( Z > p ) : p \in (0,\infty) \} < \infty$, or equivalently $\lim_{ p \to \infty} [ p \Prob( Z > p ) ] < \infty$. This condition admits any $Z$ with finite expectation, and even admits any $Z$ with a ``fat-tailed'' distribution satisfying $p^{1+\beta}\Prob( Z > p) \to 1$ as $p \to \infty$ for some $\beta > 0$. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{Local Equilibrium and the Simultaneous Stationarity Conditions}
	\label{SUBSEC:EquilibriumAndTheSSCs}
	
	The ``stationarity'' condition
	\begin{equation} 
		\label{ProfitGradientFormula}
		(\nabla_f \hat{\pi}_f)(\vec{p}) 
			= (D_f \vec{P}_f)(\vec{p})^\top (\vec{p}_f - \vec{c}_f) + \vec{P}_f(\vec{p})
			= \vec{0}
	\end{equation}
	is necessary for $\vec{p}_f \in (\vec{0},\varsigma_*\vec{1}) \subset \R^{J_f}$ to be a local maximizer of $\hat{\pi}_f(\cdot,\vec{p}_{-f}) : \set{P}^{J_f} \to \R$ when the choice probabilities $\vec{P}_f(\cdot,\vec{p}_{-f}) : \set{P}^{J_f} \to [0,1]^{J_f}$ are continuously differentiable \citep{Munkres91}. Combining the stationarity condition for each firm we obtain the {\em Simultaneous Stationarity Condition}, a necessary condition for (local) equilibrium. 
	
	\begin{proposition}[Simultaneous Stationarity Condition]
		\label{SSCProp}
		Suppose $\vec{P}$ is continuously differentiable on some open $\set{A} \subset (\vec{0},\bsym{\infty})$, and let $(\tilde{\nabla}\hat{\pi})(\vec{p})$ denote the ``combined gradient'' with components $((\tilde{\nabla}\hat{\pi})(\vec{p}))_j = (D_j\hat{\pi}_{f(j)})(\vec{p})$ where $f(j)$ is index of the firm offering product $j$. Let $(\tilde{D}\vec{P})(\vec{p}) \in \R^{J \times J}$ be the matrix of ``intra-firm'' price derivatives of the choice probabilities defined by
		\begin{equation*}
			\big( (\tilde{D}\vec{P})(\vec{p}) \big)_{j,k} 
				= \left\{ \begin{aligned}
					&(D_kP_j)(\vec{p})	&&\quad\text{if } f(j) = f(k) \\
					&\quad\quad 0		&&\quad\text{otherwise }
				\end{aligned} \right. .
		\end{equation*}
		If $\vec{p} \in \set{A}$ is a local equilibrium, then 
		\begin{equation}
			\label{SSCs}
			(\tilde{\nabla}\hat{\pi})(\vec{p})
				= (\tilde{D}\vec{P})(\vec{p})^\top (\vec{p} - \vec{c}) + \vec{P}(\vec{p}) 
				= \vec{0}. 
		\end{equation}
	\end{proposition}
	Prices $\vec{p}$ satisfying Eqn. (\ref{SSCs}) are called ``simultaneously stationary.''
	
	The necessity of the Simultaneous Stationarity Condition does not depend on the type of choice model, but only on the continuous differentiability of the choice probabilities with respect to price. Thus, Eqn. (\ref{SSCs}) has appeared in many different studies using alternative specifications for the choice probabilities including Logit, Nested Logit, and Mixed Logit models, as well as arbitrary demand functions. 
	
	Of course, simultaneously stationary prices need not be equilibria. Linking simultaneous stationarity with local optimality of profits requires verifying the second-order conditions; see Section \ref{ECSUBSEC:Sufficiency} for a derivation of the second order conditions in our case. 
	
%	For example: \cite{Besanko98} apply this condition for Logit models; \cite{Goldberg95,Goldberg98}, \cite{Besanko98}, and \cite{VillasBoas05} apply this condition for certain Generalized Extreme Value models (particularly, Nested Logit models); and \cite{Berry95,Berry04a}, \cite{Nevo00a, Nevo01}, \cite{Sudhir01}, \cite{Petrin02}, \cite{Smith04}, \cite{Thomadsen05}, and \cite{Beresteanu08} (among others) apply this for Mixed Logit models. Furthermore, this applies to an arbitrary demand function, rather than just RUMs; see, e.g., \cite{Bresnahan87, Hausman02}. 
%	
%	Of course, simultaneously stationary prices need not be equilibria. Linking simultaneous stationarity with local optimality of profits requires verifying the second-order conditions; i.e. verifying the negative-definiteness of each firm's Hessian of profits. 
	
%	In the more restrictive context of Logit models, \cite{Morrow08a} provide conditions on the utility function $u$ under which the first-order necessary condition is also sufficient. Under these conditions profit maximizing prices are unique and any simultaneously stationary prices are, in fact, an equilibrium. Conditions that generalize this result to Mixed Logit models are not yet known, but would relieve the need to numerically check the second-order conditions at simultaneously stationary prices. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{Choice Probability Derivatives}
	\label{SUBSEC:ChoiceProbabilityDerivatives}
	
	We rely on the following representation of the Mixed Logit choice probability derivatives. In what follows, $(Dw_j)(p_j)$ denotes the derivative of the price component of utility, $w_j$, with respect to price. 
	\begin{proposition}
		\label{MixedLogitDerivatives}
		Fix $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$, let $u_j$ be given as in Assumption \ref{MixedLogitUtilityAssump} for all $j$, and suppose the Leibniz Rule holds for the Mixed Logit choice probabilities; that is, $(D_k P_j)(\vec{p}) = \int (D_jP_k^L)(\bsym{\theta},\vec{p}) d\mu(\bsym{\theta})$. Then the Jacobian matrix of $\vec{P}$ is given by $(D\vec{P})(\vec{p}) = \bsym{\Lambda}(\vec{p}) - \bsym{\Gamma}(\vec{p})$ where $\bsym{\Lambda}(\vec{p}) \in \R^{J \times J}$ is the diagonal matrix with $( \bsym{\Lambda}(\vec{p}) )_{j,j} = \lambda_j(\vec{p})$ where 
		\begin{equation*}
			\lambda_j(\vec{p}) = \int_{\set{L}(p_j)} (Dw_j)(\bsym{\theta},p_j) P_j^L(\bsym{\theta},\vec{p}) d\mu(\bsym{\theta}),
			\quad\quad
			\set{L}(p) = \{ \bsym{\theta} : \varsigma(\bsym{\theta}) > p \}
		\end{equation*}
		and $\bsym{\Gamma}(\vec{p})$ is the full $J \times J$ matrix with entries
		\begin{equation*}
			\gamma_{j,k}(\vec{p}) 
				= \int_{\set{G}(p_j,p_k)} P_j^L(\bsym{\theta},\vec{p})P_k^L(\bsym{\theta},\vec{p})(Dw_k)(\bsym{\theta},p_k) d\mu(\bsym{\theta}),
			\quad\quad
			\set{G}(p,q) = \set{L}(p) \cap \set{L}(q).
		\end{equation*}
		The intra-firm price derivatives of the Mixed Logit choice probabilities are given by $(\tilde{D}\vec{P})(\vec{p}) = \bsym{\Lambda}(\vec{p}) - \tilde{\bsym{\Gamma}}(\vec{p})$ where $\big( \tilde{\bsym{\Gamma}}(\vec{p}) \big)_{j,k} = \gamma_{j,k}(\vec{p})$ if $f(j) = f(k)$ and $\big( \tilde{\bsym{\Gamma}}(\vec{p}) \big)_{j,k} = 0$ otherwise. 
%		\begin{equation*}
%			\big( \tilde{\bsym{\Gamma}}(\vec{p}) \big)_{j,k}
%				= \left\{ \begin{aligned}
%					&\gamma_{j,k}(\vec{p})	&&\quad\text{if } j,k \in \set{J}_f \text{ for some } f \\
%					&\quad 0 				&&\quad\text{otherwise }
%				\end{aligned} \right.
%		\end{equation*}
	\end{proposition}
%	$\bsym{\lambda}$ is closely related to a familiar economic quantity. Recall that the ``inclusive value,'' or expected maximum utility, conditional on demographics is given by \citep{Small81,Train03}
%	\begin{equation*}
%		\iota^L(\bsym{\theta},\vec{p}) 
%			= \log \left( e^{\vartheta(\bsym{\theta})} + \sum_{j=1}^J e^{u_j(\bsym{\theta},p_j)} \right)
%	\end{equation*}
%	It is easy to see that $\lambda_k$ is the derivative of the ``aggregate inclusive value'' $\iota(\vec{p}) = \int \iota^L(\bsym{\theta},\vec{p}) d\mu(\bsym{\theta})$ with respect to the $k\ith$ price: $\lambda_k(\vec{p}) = (D_k\iota)(\vec{p}) = \int (D_k\iota^L)(\bsym{\theta},\vec{p}) d\mu(\bsym{\theta})$. 

	Note that $\bsym{\Gamma}(\vec{p})$ and $\tilde{\bsym{\Gamma}}(\vec{p})$ are not necessarily symmetric for all $\vec{p}$. If $(Dw_k)(\bsym{\theta},p)$ is independent of both $k$ and $p$, as in the case of the \cite{Boyd80} model presented in Example \ref{BoydExample} above, then $\bsym{\Gamma}(\vec{p})$ (and thus $\tilde{\bsym{\Gamma}}(\vec{p})$) is symmetric for all $\vec{p}$. On the other hand if $(Dw_k)(\bsym{\theta},\cdot)$ is independent of $k$ and strictly monotone in $p$, as is the case of the strictly concave in price utility from \cite{Berry95}, then $\gamma_{j,k}(\vec{p}) = \gamma_{k,j}(\vec{p})$ if and only if $p_j = p_k$. 
	
%	a simple Logit model with either product-specific or nonlinear price components of utility will not have symmetric $\bsym{\Gamma}(\vec{p})$. Similarly, a full Mixed Logit model with product-specific or nonlinear price components of utility need not be symmetric. For example, 
		
	The following assumption gives a simple, abstract condition on $(\vec{u},\vartheta,\mu)$ that guarantees the Leibniz Rule holds and defines continuously differentiable choice probabilities. 
%		\begin{equation*}
%			\psi_k(\bsym{\theta},p)
%				= \left\{ \begin{aligned}
%					&\abs{(Dw_k)(\bsym{\theta},p)} \left( \frac{ e^{u_k(\bsym{\theta},p)} }{ e^{\vartheta(\bsym{\theta})} + e^{u_k(\bsym{\theta},p)} } \right)
%						&&\quad \text{if } p < \varsigma(\bsym{\theta}) \\
%					&\quad\quad\quad\quad\quad\quad 0
%						&&\quad \text{if } p \geq \varsigma(\bsym{\theta}) \\
%				\end{aligned} \right .
%		\end{equation*}
	\begin{assumption}
		\label{LeibnizRuleCondition}
		Let $k$ be arbitrary and define $\psi_k : \set{T} \times \set{P} \to \set{P}$ by 
		\begin{equation*}
			\psi_k(\bsym{\theta},p) 
				= \left\{ \begin{aligned}
					&\abs{(Dw_k)(\bsym{\theta},p)}
						\left( \frac{ e^{u_k(\bsym{\theta},p)} }
							{ e^{\vartheta(\bsym{\theta})} + e^{u_k(\bsym{\theta},p)} } \right)
					&&\quad\text{if } p < \varsigma(\bsym{\theta})\\
					&\quad\quad\quad\quad\quad
						0 &&\quad\text{if } p \geq \varsigma(\bsym{\theta})\\ 
				\end{aligned} \right .
		\end{equation*}
		Assume (i) $\psi_k(\bsym{\theta},\cdot) : (0,\varsigma_*) \to \set{P}$ is continuous for $\mu$-a.e. $\bsym{\theta} \in \set{T}$; that is, $\psi_k(\bsym{\theta},q) \to \psi_k(\bsym{\theta},p)$ as $q \to p$ for any $p \in (0,\varsigma_*)$. (ii) $\psi_k(\cdot,p^\prime) : \set{T} \to \set{P}$ is uniformly $\mu$-integrable for all $p^\prime$ in some neighborhood of any $p \in (0,\varsigma_*)$; that is, there exists some $\varphi : \set{T} \to [0,\infty)$ with $\int \varphi (\bsym{\theta}) d\mu(\bsym{\theta}) < \infty$ (that may depend on $k$ and $p$), such that $\psi_k(\bsym{\theta},p^\prime) \leq \varphi (\bsym{\theta})$ for all $p^\prime$ in some neighborhood of $p$. 
	\end{assumption}
	
	\begin{proposition}
		\label{LeibnizRule}
		If Assumption \ref{LeibnizRuleCondition} holds, then the Leibniz Rule holds for the Mixed Logit choice probabilities which are also continuously differentiable on $(\vec{0},\varsigma_*\vec{1})$. 
	\end{proposition}
	We verify Assumption \ref{LeibnizRuleCondition} directly for our example problems in Section \ref{SEC:Examples}. 
	
%	We investigate Assumption \ref{LeibnizRuleCondition} a bit further. First note that Assumption \ref{LeibnizRuleCondition}, (i) is trivial for all $\bsym{\theta}$ such that $\varsigma(\bsym{\theta}) = \infty$, given Assumption \ref{MixedLogitUtilityAssump}. Next, $\psi_k(\bsym{\theta},p)$ is continuous at all $p > \varsigma(\bsym{\theta})$ for $\mu$-a.e. $\bsym{\theta}$ with $\varsigma(\bsym{\theta}) < \infty$ by definition. Assumption \ref{MixedLogitUtilityAssump} ensures that $\psi_k(\bsym{\theta},p)$ is continuous at all $p < \varsigma(\bsym{\theta})$ for $\mu$-a.e. $\bsym{\theta}$. Thus Assumption \ref{LeibnizRuleCondition}, (i) amounts to the assumption that $\psi_k(\bsym{\theta},\cdot)$ is continuous at $\varsigma(\bsym{\theta})$, i.e. $\psi_k(\bsym{\theta},p) \to 0$ as $p \uparrow \varsigma(\bsym{\theta})$, for $\mu$-a.e. $\bsym{\theta}$. 
%%	This, in turn, amounts to the requirement that 
%%	\begin{equation*}
%%		\lim_{p \uparrow \varsigma(\bsym{\theta})} \abs{ D^p \left[ e^{w_k(\bsym{\theta},p)} \right] }
%%			= \lim_{p \uparrow \varsigma(\bsym{\theta})} \Big[ \abs{(Dw_k)(\bsym{\theta},p)}e^{w_k(\bsym{\theta},p)} \Big] = 0
%%	\end{equation*}
%%	for $\mu$-a.e. $\bsym{\theta}$. 
%	The following lemma uses this to provide a necessary and sufficient condition on $u$ to ensure Assumption \ref{LeibnizRuleCondition}, (i) holds. 
%	\begin{lemma}
%		\label{LogCondition}
%		Assumption \ref{LeibnizRuleCondition}, (i) holds if, and only if, for $\mu$-a.e. $\bsym{\theta}$ such that $\varsigma(\bsym{\theta}) < \infty$ and every $\varepsilon > 0$ there exists some $\delta(\bsym{\theta},\varepsilon) > 0$ such that $w_k(\bsym{\theta},p) \leq \log ( \varsigma(\bsym{\theta}) - p ) + \log \varepsilon$ for all $p > \varsigma(\bsym{\theta}) - \delta(\bsym{\theta},\varepsilon)$. 
%	\end{lemma}
%	
%	The choice $w_k(\bsym{\theta},p) = \alpha(\bsym{\theta}) \log ( \varsigma(\bsym{\theta}) - p )$ is a popular choice \citep{Berry95, Petrin02, Berry04a}. As can be checked, this choice violates this condition (and thus Assumption \ref{LeibnizRuleCondition}, Condition (i)) if $\alpha(\bsym{\theta}) \leq 1$, but satisfies it so long as $\alpha(\bsym{\theta}) > 1$. 

%	Next we turn to Assumption \ref{LeibnizRuleCondition}, (ii), the uniform integrability condition. Recall that the $\delta$-{\em modulus of continuity} of $\psi_k(\bsym{\theta},\cdot)$ about $p$ is defined by
%	\begin{equation*}
%		\omega_p^\delta(\bsym{\theta})
%			= \sup \Big\{ \abs{ \psi_k(\bsym{\theta},p) - \psi_k(\bsym{\theta},q) } : \abs{ p - q } \leq \delta \Big \}. 
%	\end{equation*}
%	
%	\begin{lemma}
%		Assumption \ref{LeibnizRuleCondition}, (ii) holds if, and only if, there exists some $\delta > 0$ such that $\psi_k(\cdot,p) : \set{T} \to \set{P}$ and $\omega_p^\delta : \set{T} \to \set{P}$ are $\mu$-integrable. 
%	\end{lemma}
%	Existence of {\em some} $\delta > 0$ is sufficient because $\omega_p^\delta$ is non-increasing in $\delta$. 
%	
%	How does this Lemma change our characterization of the Leibniz rule? 
%	  
%%	\begin{equation*}
%%		\sup \Big\{ \abs{ \psi_k(\bsym{\theta},p) - \psi_k(\bsym{\theta},q) } : \abs{ p - q } \leq \delta \Big \}
%%			\geq \sup \Big\{ \abs{ \psi_k(\bsym{\theta},p) - \psi_k(\bsym{\theta},q) } : \abs{ p - q } \leq \delta^\prime \Big \}
%%	\end{equation*}
%%	whenever $\delta \geq \delta^\prime$. 
	
	We close this section by stating some basic results concerning $(\tilde{D}\vec{P})(\vec{p})$ that are used below. 
	\begin{lemma}
		\label{LamGamLemma}
		Let $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$,  suppose $\vartheta : \set{T} \to (-\infty,\infty)$, and define
		\begin{equation}
			\label{OmegaDef}
			\bsym{\Omega}_f(\vec{p}) = \bsym{\Lambda}_f(\vec{p})\inv \bsym{\Gamma}_f(\vec{p})^\top
			\quad\quad\text{and}\quad\quad
			\tilde{\bsym{\Omega}}(\vec{p}) = \bsym{\Lambda}(\vec{p})\inv \tilde{\bsym{\Gamma}}(\vec{p})^\top. 
		\end{equation}
		\begin{itemize}
		
			\item[(i)] $(D_f\vec{P}_f)(\vec{p})^\top = \bsym{\Lambda}_f(\vec{p}) ( \vec{I} - \bsym{\Omega}_f(\vec{p}) )$ and $(\tilde{D}\vec{P})(\vec{p})^\top = \bsym{\Lambda}(\vec{p}) ( \vec{I} - \tilde{\bsym{\Omega}}(\vec{p}) )$. 
			
			\item[(ii)] $\norm{ \bsym{\Omega}_f(\vec{p}) }_\infty < 1$ and $\norm{ \tilde{\bsym{\Omega}}(\vec{p}) }_\infty < 1$. 
			
			\item[(iii)] The matrices $\vec{I} - \bsym{\Omega}_f(\vec{p}) \in \R^{J_f \times J_f}$ and $\vec{I} - \tilde{\bsym{\Omega}}(\vec{p}) \in \R^{J \times J}$ are strictly diagonally dominant and nonsingular. Subsequently $(D_f\vec{P}_f)(\vec{p})^\top$ and $(\tilde{D}\vec{P})(\vec{p})^\top$ are strictly diagonally dominant and nonsingular. 
			
			\item[(iv)] $(\vec{I} - \bsym{\Omega}_f(\vec{p}))\inv \in \R^{J_f \times J_f}$ and $(\vec{I} - \tilde{\bsym{\Omega}}(\vec{p}))\inv \in \R^{J \times J}$ map positive vectors to positive vectors. 
		\end{itemize}
	\end{lemma}
	
%	\begin{lemma}
%		\label{LamGamLemma}
%		Let $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$ and suppose $\vartheta : \set{T} \to (-\infty,\infty)$. Define $\bsym{\Omega}_f(\vec{p}) = \bsym{\Lambda}_f(\vec{p})\inv \bsym{\Gamma}_f(\vec{p})^\top$ and $\bsym{\Omega}(\vec{p}) = \bsym{\Lambda}(\vec{p})\inv \tilde{\bsym{\Gamma}}(\vec{p})^\top$. Then the following hold: (i) $\norm{ \bsym{\Omega}_f(\vec{p}) }_\infty < 1$ and $\norm{ \bsym{\Omega}(\vec{p}) }_\infty < 1$. (ii) The matrices $\vec{I} - \bsym{\Omega}_f(\vec{p}) \in \R^{J_f \times J_f}$ and $\vec{I} - \bsym{\Omega}(\vec{p}) \in \R^{J \times J}$ are strictly diagonally dominant and nonsingular. Subsequently $(\tilde{D}\vec{P})(\vec{p})^\top = \bsym{\Lambda}(\vec{p})( \vec{I} - \bsym{\Omega}(\vec{p}) )$ is strictly diagonally dominant and nonsingular. (iii) $(\vec{I} - \bsym{\Omega}_f(\vec{p}))\inv \in \R^{J_f \times J_f}$ and $(\vec{I} - \bsym{\Omega}(\vec{p}))\inv \in \R^{J \times J}$ map positive vectors to positive vectors. 
%	\end{lemma}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{The Markup Equation}
	\label{SUBSEC:MarkupEqn}
	
	In most existing empirical studies, Eqn. (\ref{SSCs}) has been used through the corresponding {\em markup equation} $\vec{p} = \vec{c} + \bsym{\eta}(\vec{p})$ where $\bsym{\eta} : (\vec{0},\varsigma_*\vec{1}) \to \R^J$ is defined by
	\begin{equation}
		\label{MarkupEquation}
		\bsym{\eta}(\vec{p}) 
			= - (\tilde{D}\vec{P})(\vec{p})^{-\top} \vec{P}(\vec{p}). 
	\end{equation}
	Lemma \ref{LamGamLemma}, claim (iii), proves that $(\tilde{D}\vec{P})(\vec{p})^\top$ is nonsingular for the class of Mixed Logit models generated by Assumptions \ref{MixedLogitUtilityAssump} and \ref{LeibnizRuleCondition}, and thus $\bsym{\eta}$ is well-defined. We also note that there is a simple relationship between $\bsym{\eta}$ and the combined gradient: 
	\begin{equation}
		\label{Eta-CGRelation}
		(\tilde{\nabla}\hat{\pi})(\vec{p}) 
			= (\tilde{D}\vec{P})(\vec{p})^{\top}(\vec{p}-\vec{c}-\bsym{\eta}(\vec{p})). 
	\end{equation}
	
	Traditionally, the markup equation has been used to estimate {\em costs} assuming {\em observed} prices are in equilibrium via the formula $\vec{c} = \vec{p} - \bsym{\eta}(\vec{p})$; see, e.g., \cite{Berry95}. These cost estimates often form the basis of counterfactual experiments with an estimated demand model. \cite{Beresteanu08} have recently suggested that the markup equation is also useful for computing equilibrium prices, a suggestion we explore further below. Note that the markup equation must be understood as a nonlinear fixed-point equation when applied to compute equilibrium prices. 
	
	Several important properties of $\bsym{\eta}$ are derived from an alternative form of Eqn. (\ref{MarkupEquation}) based on Lemma \ref{LamGamLemma}:
	\begin{equation}
		\label{EtaEqn}
		\Big( \vec{I} - \tilde{\bsym{\Omega}}(\vec{p}) \Big) 
				\bsym{\eta}(\vec{p})
			= - \bsym{\Lambda}(\vec{p})\inv\vec{P}(\vec{p}).
	\end{equation} 
	First, this form proves that profit-optimal markups are positive for the class of Mixed Logit models we consider, thanks to Lemma \ref{LamGamLemma}, claim (iv).  
	\begin{lemma}
		\label{PositiveMixedLogitMarkups}
		$\bsym{\eta}(\vec{p}) > \vec{0}$ for all $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$. Hence if $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$ is a local equilibrium, then $\vec{p} > \vec{c}$. 
	\end{lemma}
	Second, Eqn. (\ref{EtaEqn}) is better conditioned than Eqn. (\ref{MarkupEquation}), and thus should be used to actually compute $\bsym{\eta}$; see the E-Companion, Section \ref{ECSUBSEC:CompBurden}. Third, Eqn. (\ref{EtaEqn}) also provides bounds on the magnitude of values taken by $\bsym{\eta}$:
	\begin{lemma} 
		For all $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$, $\bsym{\eta}$ satisfies
		\begin{equation}
			\label{EtaBounds}
			\frac{ \norm{ \bsym{\Lambda}(\vec{p})\inv\vec{P}(\vec{p}) }_\infty }
							{ 1 + \norm{ \tilde{\bsym{\Omega}}(\vec{p}) }_\infty }
					\leq \norm{ \bsym{\eta}(\vec{p}) }_\infty
					\leq \frac{\norm{\bsym{\Lambda}(\vec{p})\inv\vec{P}(\vec{p})}_\infty}
							{1 - \norm{\tilde{\bsym{\Omega}}(\vec{p})}_\infty}. 
		\end{equation}
	\end{lemma}
	The upper bound suggests the following assumptions to ensure that $\bsym{\eta}$ itself is bounded:
	\begin{assumption}
		\label{BoundedAssumption}
		Suppose $\varsigma_* = \infty$ and there exist $M > 0$ and $\varepsilon \in (0,1)$ such that
		\begin{align}
			\label{LPBound}
			\sup \big\{ \norm{ \bsym{\Lambda}(\vec{p})\inv\vec{P}(\vec{p}) }_\infty \; : \; \vec{p} \in \set{P}^J \big\} &\leq M \\
			\label{LGBound}
			\sup \big\{ \norm{\bsym{\Omega}(\vec{p})}_\infty \; : \; \vec{p} \in \set{P}^J \big\}
				&= 1 - \varepsilon. 
		\end{align}
	\end{assumption}
	
	\begin{lemma}
		\label{BoundedEta}
		If Assumption \ref{BoundedAssumption} holds then $N = \sup \{ \norm{ \bsym{\eta}(\vec{p}) }_\infty : \vec{p} \in \set{P}^J \} < \infty$. Moreover Eqn. (\ref{LPBound}) in Assumption \ref{BoundedAssumption} is necessary for $N$ to be finite. 
	\end{lemma}
%	If $\bsym{\eta}$ is bounded and $\varsigma_* = \infty$, $\vec{p} - \vec{c} - \bsym{\eta}(\vec{p})$ is norm-coercive (see Lemma \ref{Coercivity}). This property is important for effective applications of Newton's method. 

	Under simple Logit, $P_k^L(\vec{p})/\abs{\lambda_k(\vec{p})} = \abs{(Dw_k)(p_k)}\inv$ and $\bsym{\Omega}_f(\vec{p}) = \vec{1}\vec{P}_f^L(\vec{p})^\top$. Thus Eqn. (\ref{LPBound}) is akin to concavity of $w_k$ for all sufficiently large $p_k$, and Eqn. (\ref{LGBound}) is implied by $\vartheta > -\infty$, i.e. the existence of an outside good with positive purchase probability.  
	
	Lemma \ref{BoundedEta} enables a proof of the existence of finite simultaneously stationary prices. 
	\begin{corollary}
		\label{Existence}
		If Assumption \ref{BoundedAssumption} holds then there exists at least one vector of finite simultaneously stationary prices. 
	\end{corollary}
	This is a direct consequence of Brower's fixed-point theorem. Corollary \ref{Existence} does not, however, establish the existence of a local {\em equilibrium}, or the uniqueness of simultaneously stationary points. To address the former will require additional conditions to ensure that each firm's profits are locally concave at the simultaneously stationary prices whose existence Corollary \ref{Existence} ensures. 
	
%	This additional step has traditionally been made for single-product firms by using quasi-concavity of profits \citep{Caplin91}. Unfortunately this property does not hold for multi-product firms \citep{Hanson96}, even under simple Logit. For multi-product firms and the Logit model, \cite{Morrow08a} use a direct analysis of the second-order conditions at any stationary point and the Poincare-Hopf Theorem \citep{Milnor65, Simsek07} to overcome the lack of quasi-concavity in multi-product firm profits. A similar analysis may prove fruitful for some Mixed Logit models. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{Another Fixed-Point Equation}
	\label{SUBSEC:ZetaMap}
	
	We now derive our second fixed-point representation of equilibrium. The markup equation $\vec{p} = \vec{c} + \bsym{\eta}(\vec{p})$ can be re-arranged to obtain the equivalent expression $\vec{p} = \vec{c} + \bsym{\zeta}(\vec{p})$ where $\bsym{\zeta} : (\vec{0},\varsigma_*\vec{1}) \to \R^J$ is defined by
	\begin{equation}
		\label{MixedLogitFPEEqn}
		\bsym{\zeta}(\vec{p}) = \tilde{\bsym{\Omega}}(\vec{p})(\vec{p} - \vec{c}) - \bsym{\Lambda}(\vec{p})\inv\vec{P}(\vec{p}). 
	\end{equation}
	This can be thought of as separating the effects of the identity ($\vec{I}$) and contractive ($\tilde{\bsym{\Omega}}(\vec{p})$) parts of the system defining simultaneously stationary prices, much like the Jacobi iteration for linear systems. Alternatively, the equation
	\begin{equation}
		\label{Zeta-CGRelation}
		(\tilde{\nabla}\hat{\pi})(\vec{p}) = \bsym{\Lambda}(\vec{p})(\vec{p}-\vec{c}-\bsym{\zeta}(\vec{p})). 
	\end{equation}
	illustrates that this can also be viewed as factoring out $\bsym{\Lambda}(\vec{p})$, the gradient of the aggregate inclusive value, from the combined gradient. 
	
	Unlike $\bsym{\eta}$, it is not obvious whether $\bsym{\zeta}$ is bounded. However Assumption \ref{BoundedAssumption} still defines $\bsym{\zeta}$'s asymptotic properties. 
	\begin{lemma}
		\label{ZetaGrowth}
		Under Assumption \ref{BoundedAssumption} $\norm{\bsym{\zeta}(\vec{p})}_\infty < \norm{\vec{p}-\vec{c}}_\infty$ whenever $\norm{\vec{p}-\vec{c}}_\infty > M / \varepsilon$. Moreover $\norm{\vec{p}-\vec{c}}_\infty - \norm{\bsym{\zeta}(\vec{p})}_\infty \to \infty$ as $\norm{ \vec{p} - \vec{c} }_\infty \to \infty$. 
%		\begin{equation*}
%			\norm{\vec{p}-\vec{c}}_\infty - \norm{\bsym{\zeta}(\vec{p})}_\infty \to \infty
%			\quad\quad\text{as}\quad\quad
%			\norm{ \vec{p} - \vec{c} }_\infty \to \infty. 
%		\end{equation*}
	\end{lemma}
%	This result can be used to show that $\vec{p} - \vec{c} - \bsym{\zeta}(\vec{p})$ is norm-coercive (see Lemma \ref{Coercivity}). 
	
%	\cite{Morrow08a} use a slightly different set of assumptions for their analysis of equilibrium prices under Logit: 
%	\begin{assumption}
%		Suppose $\varsigma_* = \infty$. (i) For all $k$ there exists some $s_k < 1$ and $\bar{p}_k > 0$ such that $P_k(\vec{p})/\abs{\lambda_k(\vec{p})} < s_k p_k$ for all $p_k > \bar{p}_k$. (ii) For all $f$ and all $k \in \set{J}_f$, $\abs{\lambda_k(\vec{p})}\inv\sum_{j \in \set{J}_f} \gamma_{j,k}(\vec{p})(p_j-c_j) \to 0$ as $p_k \to \infty$. 
%	\end{assumption}
%	Assumption (i) is generally weaker than Eqn. \ref{LPBound} in Assumption \ref{BoundedAssumption}, but at least for Logit models, is strictly weaker only if $\abs{(Dw_k)(p_k)} \to 0$ as $p_k \to \infty$; i.e. utility is eventually convex. On the other hand Assumption (ii) is stronger than Eqn. \ref{LGBound} in Assumption \ref{BoundedAssumption}, which only implies that
%	\begin{equation*}
%		\norm{\bsym{\Lambda}(\vec{p})\inv\tilde{\bsym{\Gamma}}(\vec{p})^\top(\vec{p}-\vec{c})}_\infty
%			\leq \norm{\bsym{\Lambda}(\vec{p})\inv\tilde{\bsym{\Gamma}}(\vec{p})^\top}_\infty\norm{(\vec{p}-\vec{c})}_\infty
%			\leq (1 - \varepsilon ) \norm{(\vec{p}-\vec{c})}_\infty
%	\end{equation*}
%	For Logit models $\abs{\lambda_k(\vec{p})}\inv\sum_{j \in \set{J}_f} \gamma_{j,k}(\vec{p})(p_j-c_j) = \hat{\pi}_f^L(\vec{p})$ for all $k$, and a weak assumption on the utility function ensures that profits vanish as prices tend to infinity \citep{Morrow08a}. 
%	
%	These revised assumptions imply that 
	
	We close this section with a relationship between the maps $\bsym{\zeta}$ and $\bsym{\eta}$. 
	\begin{proposition}
		\label{ZetaEtaDistinct}
		For any $\vec{p} \in (\vec{0},\varsigma_*\vec{1})$, $\bsym{\zeta}(\vec{p}) = \tilde{\bsym{\Omega}}(\vec{p})(\vec{p} - \vec{c}) + ( \vec{I} - \tilde{\bsym{\Omega}}(\vec{p}) ) \bsym{\eta}(\vec{p})$. 
%		\begin{align*}
%			\bsym{\zeta}(\vec{p})
%				&= \bsym{\Omega}(\vec{p})(\vec{p} - \vec{c})
%					+ ( \vec{I} - \bsym{\Omega}(\vec{p}) ) \bsym{\eta}(\vec{p}) \\
%			\vec{c} + \bsym{\zeta}(\vec{p})
%				&= \bsym{\Omega}(\vec{p})\vec{p}
%					+ ( \vec{I} - \bsym{\Omega}(\vec{p}) )
%						( \vec{c} + \bsym{\eta}(\vec{p}) ) \\
%			\vec{p} - \vec{c} - \bsym{\zeta}(\vec{p})
%				&= ( \vec{I} - \bsym{\Omega}(\vec{p}) )( \vec{p} - \vec{c} - \bsym{\eta}(\vec{p}) ). 
%		\end{align*}
	\end{proposition}
	This equation, which follows directly from Eqns. (\ref{EtaEqn}) and (\ref{MixedLogitFPEEqn}), implies that $\bsym{\zeta}(\vec{p}) = \bsym{\eta}(\vec{p})$ if, and only if, $\vec{p} - \vec{c} - \bsym{\eta}(\vec{p}) = \vec{p} - \vec{c} - \bsym{\zeta}(\vec{p})$ lie in the null space of $\tilde{\bsym{\Omega}}(\vec{p})$. Thus if $\tilde{\bsym{\Omega}}(\vec{p})$ is full-rank, $\bsym{\zeta}$ and $\bsym{\eta}$ coincide {\em only} at simultaneously stationary prices. Simple examples of Mixed Logit models can be constructed that always have $\mathrm{rank} \; \tilde{\bsym{\Omega}}(\vec{p}) = J$. For Logit, $\bsym{\Omega}_f(\vec{p}) = \vec{1}\vec{P}_f^L(\vec{p})^\top$ for all $f$ and $\tilde{\bsym{\Omega}}(\vec{p})$ always has rank $F \leq J$. However the analysis in \cite{Morrow08a} can be used to show that $\bsym{\zeta}$ and $\bsym{\eta}$ coincide only at simultaneously stationary prices. In so far as $\bsym{\eta}$ and $\bsym{\zeta}$ are distinct maps, they can generate numerical methods for the computation of equilibrium prices with entirely different properties. 
	
%	As a consequence of (ii) numerical methods based on $\bsym{\zeta}$ and $\bsym{\eta}$ can, in principle, have entirely different properties. 

	\subsection{Coercivity}
	
	
	\begin{assumption}
		\label{LVA}
		Let $\psi_k$ be defined as in Assumption \ref{LeibnizRuleCondition}. (i) $p_k \psi_k(\bsym{\theta},p_k) \to 0$ as $p_k \uparrow \varsigma(\bsym{\theta})$ for $\mu$-a.e. $\bsym{\theta}$. (ii) There exists $M < \infty$ and $\bar{p}_k \in [0,\varsigma_*)$ such that $p_k \int \psi_k(\bsym{\theta},p_k) d\mu(\bsym{\theta}) \leq M$ for all $p_k \in (\bar{p}_k,\varsigma_*)$. 
%		\begin{itemize}
%			\item[(i)] $p_k \psi_k(\bsym{\theta},p_k) \to 0$ as $p_k \uparrow \varsigma(\bsym{\theta})$ for $\mu$-a.e. $\bsym{\theta}$ and 
%			\item[(ii)] there exists $M < \infty$ and $\bar{p}_k \in [0,\varsigma_*)$ such that $p_k \int \psi_k(\bsym{\theta},p_k) d\mu(\bsym{\theta}) \leq M$ for all $p_k \in (\bar{p}_k,\varsigma_*)$. 
%%			\begin{equation*}
%%				p_k \int \psi_k(\bsym{\theta},p_k) d\mu(\bsym{\theta})
%%%					= \int_{ \{ \bsym{\theta} : \varsigma(\bsym{\theta}) > p_k \} } \abs{(Dw_k)(\bsym{\theta},p_k)} e^{ u_k(\bsym{\theta},p_k) - \vartheta(\bsym{\theta}) } d\mu(\bsym{\theta})
%%					\leq M. 
%%			\end{equation*}
%		\end{itemize}
	\end{assumption}
	As with Assumption \ref{LeibnizRuleCondition} above, (i) and (ii) are essentially conditions for the Dominated Convergence Theorem. Note that if $\varsigma(\bsym{\theta}) < \infty$ then (i) holds if, and only if, $\psi_k(\bsym{\theta},p_k) \to 0$ as $p_k \uparrow \varsigma(\bsym{\theta})$; i.e. $\psi_k(\bsym{\theta},\cdot)$ is continuous at $\varsigma(\bsym{\theta})$. Thus if $\varsigma(\bsym{\theta}) < \infty$ Assumption \ref{LVA}, (i), and Assumption \ref{LeibnizRuleCondition}, (i) coincide. 
	
	\begin{lemma}
		\label{LambdaVanishes}
		If Assumption \ref{LVA} holds then $p_k \abs{ \lambda_k(\vec{p}) } \to 0$ as $p_k \to \varsigma_*$ for all $k$. Additionally, $p_k \abs{ \gamma_{j,k}(\vec{p}) } \to 0$ as $p_k \to \varsigma_*$ for all $j,k$. Subsequently, $(D_k\hat{\pi}_{f(k)})(\vec{p}) \to 0$ as $p_k \to \varsigma_*$. 
	\end{lemma}
	
	In other words, under Assumption \ref{LVA} components of $\vec{F}_\pi$ vanish as the corresponding price tends to $\varsigma_*$ {\em even though this may not mean that these prices maximize profits}. Because of this, CG-NM may converge to a zero of $\vec{F}_\pi$ at $\varsigma_*\vec{1}$, or with some components equal to $\varsigma_*$, that is {\em not} an equilibrium. Because $\vec{F}_\pi(\vec{p}) \to \vec{0}$ over some divergent sequences, standard global convergence strategies based on minimizing $\norm{\vec{F}_\pi(\vec{p})}_2$ will not be effective ways of avoiding this behavior. As in Example \ref{SimpleExample}, the formulation is the problem.
	
	\begin{lemma}
		\label{Coercivity}
		If Assumption \ref{BoundedAssumption} holds, then 
		\begin{equation*}
			\lim_{\norm{\vec{p}}_\infty \to \infty} \norm{ \vec{p} - \vec{c} - \bsym{\eta}(\vec{p}) }_\infty 
				= \lim_{\norm{\vec{p}}_\infty \to \infty} \norm{ \vec{p} - \vec{c} - \bsym{\zeta}(\vec{p}) }_\infty
				= \infty. 
		\end{equation*}
%		(i) $\lim_{\norm{\vec{p}}_\infty \to \varsigma_*} \norm{ \vec{p} - \vec{c} - \bsym{\eta}(\vec{p}) }_\infty > 0$ and $\lim_{\norm{\vec{p}}_\infty \to \varsigma_*} \norm{ \vec{p} - \vec{c} - \bsym{\zeta}(\vec{p}) }_\infty > 0$. 
%		(ii) If $\varsigma_* = \infty$, $\lim_{\norm{\vec{p}}_\infty \to \infty} \norm{ \vec{p} - \vec{c} - \bsym{\eta}(\vec{p}) }_\infty = \infty = \lim_{\norm{\vec{p}}_\infty \to \infty} \norm{ \vec{p} - \vec{c} - \bsym{\zeta}(\vec{p}) }_\infty$. 
	\end{lemma}
	By bounding the level sets of $\norm{\vec{F}(\vec{p})}_2$, this $\infty$-norm coercivity provides more confidence in applications of Newton methods with global convergence strategies that attempt to minimize $\norm{\vec{F}(\vec{p})}_2$. At least when $\varsigma_* = \infty$, iterates of such methods cannot diverge to a solution with some infinite components that is not an equilibrium. This is not to say that $\bsym{\eta}$-NM or $\bsym{\zeta}$-NM should be expected to perform perfectly. By using these transformations we have only excised the tendency for Newton's method to compute ``spurious'' solutions at infinity. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	

==> additionaldetails.tex <==

\section{Additional Details Regarding the Numerical Examples}
\label{ECSEC:AdditionalDetails}

	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	\subsection{The Two Demand Models}
	\label{ECSUBSEC:DemandModels}
	
	To characterize demand for new vehicles, we employ modified versions of two existing models of new vehicle purchasing \citep{Boyd80,Berry95}. Here we give a brief description of the versions of these models used in our examples below. Random coefficient distributions are described by the parameters given in Tables \ref{TAB:BM80Coeffs} and \ref{TAB:BLP95Coeffs}. 
	
	The utility function in the \cite{Boyd80} model is linear in characteristics and price with lognormally distributed ``unobserved'' demographic variables (random coefficients) $\bsym{\theta}$, has no ``observed'' demographic variables, and does not model an outside good (i.e., $\vartheta(\bsym{\theta}) \equiv -\infty$). Specifically, with $\bsym{\theta} = (\alpha,\bsym{\beta}) \in \set{P} \times \R^3$, 
	 \begin{equation*}
	 	u(\alpha,\bsym{\beta},\vec{x},p) 
			= - \alpha p + \bsym{\beta}^\top\vec{x}
			= - \alpha p + \beta_1 x_1 + \beta_2 x_2 - \beta_3 x_3
	 \end{equation*}
	 We include the vehicle characteristics 
	 \begin{itemize}
	 	\item $x_1$: ``size'' (length times width over height, all in inches),
		\item $x_2$: ``acceleration'' (60 divided by the 0-60 acceleration time, in seconds), and 
		\item $x_3$: ``fuel consumption'' (100 times fuel consumption, in gallons per mile). 
	\end{itemize}
	A simple function of horsepower to weight ratio approximates 0-60 acceleration, a commonly used proxy in econometric models of the vehicle market. Due to a lack of data, we exclude several consumer reports ratings (``ride,'' ``handling,'' and ``noise'') used in the original model. We use 1980 USD as our monetary units. 
	
	The utility function in the \cite{Berry95} model is linear in characteristics with independent and normally distributed ``unobserved'' demographics (random coefficients), nonlinear in income minus price, and models an outside good. Specifically, with $\bsym{\theta} = (\phi,\bsym{\beta},\beta_0) \in \set{P} \times \R^3 \times \R$, 
	 \begin{equation*}
	 	% \label{BLPTypeUtility}
	 		u(\phi,\bsym{\beta},\beta_0,\vec{x},p) 
				= \alpha \log( \phi - p ) + \bsym{\beta}^\top\vec{x}
			\quad\quad\text{and}\quad\quad
			\vartheta(\phi,\bsym{\psi},\nu) = \alpha \log \phi + \beta_0
	 \end{equation*}
	 for a price coefficient $\alpha = 43.501 > 1$, income $\phi$, and random coefficients $\bsym{\beta}$. Consistent with the original model, we take income, price, and cost to be in thousands of 1983 USD where income is lognormally distributed with a log-mean of $10 - 3 \log 10 \approx 3.092$ and a log-standard deviation of 1 \citep{CPS05}. For vehicle characteristics we include 
	 \begin{itemize}
	 	\item $x_1$: operating cost (in 10 mile increments driven per dollar spent using a fuel price of 2.50 2005 USD = 1.27 1983 USD), 
		\item $x_2$: horsepower to weight ratio (weight is in 10 lbs.), and 
		\item $x_3$ length times width (both in hundreds of inches). 
	\end{itemize}
	We effectively exclude a dummy variable for standard air conditioning present in the original model by assuming standard air conditioning on all vehicles (the utility value for this is absorbed into the utility of the outside good). No other characteristics from the original model differ in our version. The random coefficients $\bsym{\beta}$ and $\beta_0$ are independently normally distributed with means and standard deviations listed in Table \ref{TAB:BLP95Coeffs}. 
	 
	 \begin{table}
	 	\TABLE
		{Coefficients describing the (lognormal) distribution of the random coefficients Mixed Logit model estimated by \cite{Boyd80}. \label{ECTAB:BM80Coeffs}}
	 	{\begin{tabular}{rcccc}
						& $\alpha$ & $\beta_1$ 	& $\beta_2$ 	& $\beta_3$	\\ \hline
			log-mean		& -7.96	& 0.589		& -1.75		& -1.28 		\\
			log-std. dev. 	& 1.18	& 0.622		& 1.34		& 0.001		\\ \hline
			\\
		\end{tabular}}
		{}
	\end{table}
	
	 \begin{table}
	 	\TABLE
		{Coefficients describing the (normal) distribution of the random coefficients Mixed Logit model estimated by \cite{Berry95}. $\phi$ is lognormally distributed, and thus reported values are the log-mean and log-standard deviation. \label{ECTAB:BLP95Coeffs}}
		{\begin{tabular}{rcccccc}
					& $\alpha$ 	& $\phi$ 	& $\beta_1$ 	& $\beta_2$ 	& $\beta_3$	& $\beta_0$ \\ \hline
			mean	& 43.501		& 10		& -0.122		& 3.460		& 2.883		& -8.582 \\
			std. dev.	& $-$		& 1		& 1.05		& 2.056		& 4.628		& 1.794 \\ \hline
		\end{tabular}}
		{}
	\end{table}
	 
	 
	 \begin{proposition}
	 	\label{BMandBLPFunctions} 
		\begin{itemize}
			\item[(i)] Assumption \ref{MixedLogitUtilityAssump} holds for both the \cite{Boyd80} and \cite{Berry95} models. 
			\item[(ii)] The conclusions of Proposition \ref{LeibnizRule} hold under the \cite{Boyd80} model. Assumption \ref{LeibnizRuleCondition}, and hence the conclusions of Proposition \ref{LeibnizRule}, hold under the \cite{Berry95} model so long as $\alpha > 1$. 
		\end{itemize}
	 \end{proposition}
	 \begin{remark}
	 We treat the \citeauthor{Boyd80} model separately because it does not have an outside good, and hence does not match the format of Assumption \ref{LeibnizRuleCondition}. The requirement that $\alpha > 1$ under the \citeauthor{Berry95} model ensures the continuously differentiability of $P_j^L(\phi,\bsym{\beta},\vec{p})$ at $p_j = \phi$. 
	 \end{remark}
	 
	\proof{Proof:}
		
		The \cite{Boyd80} model takes 
		\begin{align*}
		 	w(\alpha,\bsym{\beta},\vec{x},p) 	
				= - \alpha p
			\quad \quad\text{and}\quad \quad
			v(\alpha,\bsym{\beta},\vec{x}) 	
				= \bsym{\beta}^\top\vec{x}
		 \end{align*}
		 with no outside good. As mentioned above, $\abs{(D_kP_j^L)(\bsym{\theta},\vec{p})} \leq \abs{(Dw_k)(\bsym{\theta},p_k) }$ always holds. While this is not useful in general, it can be applied here to derive $\abs{(D_kP_j^L)(\alpha,\bsym{\beta},\vec{p})} \leq \alpha$, a bound that demonstrates the uniform $\mu$-integrability of the choice probability derivatives for any probability measure $\mu$ giving a finite expected price coefficient. Thus the conclusions of Proposition \ref{LeibnizRule} hold, since there is a finite expected price coefficient under the \citeauthor{Boyd80} model. 
	
		The \cite{Berry95} model takes $\bsym{\theta} = (\phi,\bsym{\beta},\beta_0)$ and
		\begin{align*}
		 	w(\phi,\bsym{\beta},\beta_0,\vec{x},p) 		
				= \alpha \log( \phi - p ), 
			\quad\quad
			v(\phi,\bsym{\beta},\beta_0,\vec{x},p) 
				= \bsym{\beta}^\top\vec{x},
			\quad\quad\text{and}\quad\quad
			\vartheta(\phi,\bsym{\beta},\beta_0) 
				= \alpha \log( \phi ) + \beta_0. 
		\end{align*}
		The hypothesis of Proposition \ref{LeibnizRule} is not satisfied if $\alpha < 1$: For all $\phi > p$, we have
		\begin{align*}
		 	\abs{(Dw)(\bsym{\theta},\vec{x},p)} e^{ u(\bsym{\theta},\vec{x},p) - \vartheta(\bsym{\theta}) }
			 	&= \alpha \left( \frac{1}{\phi} \right)^\alpha \left( \frac{1}{\phi-p} \right)^{1-\alpha} e^{\bsym{\beta}^\top\vec{x} - \beta_0}
		\end{align*}
		which is not $\mu$-integrable at $\phi = p$, for any $p > 0$, for any probability measure $\mu$ supported on a subset of $[0,\infty)$. By assuming $\alpha > 1$ we have instead
		\begin{align*}
		 	\abs{(Dw)(\bsym{\theta},\vec{x},p)} e^{ u(\bsym{\theta},\vec{x},p) - \vartheta(\bsym{\theta}) }
			 	&= \alpha \left( \frac{1}{\phi} \right)^\alpha \left( \phi - p \right)^{\alpha-1} e^{\bsym{\beta}^\top\vec{x} - \beta_0}
		\end{align*}
		which $\mu$-integrable for any probability measure $\mu$ supported on a subset of $[0,\infty)$. 
		
		In addition, $\abs{(Dw)(\bsym{\theta},\vec{x},p)} e^{ u(\bsym{\theta},\vec{x},p) - \vartheta(\bsym{\theta}) }$ vanishes as $\phi \downarrow p$. Thus we set 
		\begin{align*}
		 	\abs{(Dw)(\bsym{\theta},\vec{y},p)} e^{ u(\bsym{\theta},\vec{x},p) - \vartheta(\bsym{\theta}) }
				= \varphi_p(\phi)e^{\bsym{\beta}^\top\vec{x} - \beta_0}
		\end{align*}
		where now
		\begin{align*}
		 	\varphi_p(\phi)
				= \left\{ \begin{aligned}
					&\alpha \left( \frac{(\phi - p)^{\alpha - 1}}{\phi^\alpha} \right)
						&&\quad\text{if } \phi > p \\
					&\quad\quad\;\; 0 &&\quad\text{if } \phi \leq p
				\end{aligned} \right.
		\end{align*}
		We can take $\mu = \mu_\phi \times \mu_\beta$ where $\mu_p$ is a measure for $\phi$ giving it a lognormal distribution and $\mu_\beta$ is a measure for $(\bsym{\beta},\beta_0)$ giving it a normal distribution. By Fubini's theorem, 
		 \begin{align*}
		 	&\int \abs{(Dw)(\bsym{\theta},\vec{x},p)} e^{ u(\bsym{\theta},\vec{x},p) - \vartheta(\bsym{\theta}) } d\mu(\bsym{\theta}) \\
			&\quad\quad
				= \int \int \varphi_p(\phi) d\mu_\phi(\phi) \; e^{\bsym{\beta}^\top\vec{x} - \beta_0} d\mu_\beta(\bsym{\beta},\beta_0) \\
			&\quad\quad
				= \left( \int e^{\bsym{\beta}^\top\vec{x} - \beta_0} d\mu_\beta(\bsym{\beta},\beta_0) \right)
					\int \varphi_p(\phi) d\mu_\phi(\phi)
		\end{align*}
		The normal distribution on $(\bsym{\beta},\beta_0)$ ensures that
		\begin{align*}
		 	\int e^{\bsym{\beta}^\top\vec{x} - \beta_0} d\mu_\beta(\bsym{\beta},\beta_0) < \infty. 
		\end{align*}
		We turn to the price term, $\int \varphi_p(\phi) d\mu_p(\phi)$. If $p \leq p^\prime$, then $\varphi_p(\phi) \geq \varphi_{p^\prime}(\phi)$ for all $\phi$. Thus, $\varphi_p(\phi) \leq \varphi_0(\phi)$ for all $\phi$ and any $p > 0$. Now $\varphi_0(\phi) = \alpha \phi^{\alpha - 2}$, an integrable function with respect to the measure $\mu_p$ for any $\alpha > 1$. Hence $\abs{(Dw)(\bsym{\theta},\vec{y},p)} e^{ u(\bsym{\theta},\vec{y},p) - \vartheta(\bsym{\theta}) } $ is uniformly $\mu$-integrable in a neighborhood of $p$, for any $p > 0$. \Halmos
		
	\endproof
	
	\subsection{Extrapolation of Costs}
	\label{ECSUBSEC:Extrapolation}
	
	Section \ref{SUBSEC:Sensitivity} considers a differentiated product market model with 5,298 vehicles derived from the Ward's data. To generate this larger problem we extrapolate the J. D. Power cost data by assuming that variation in dealer costs is reflected in the MSRP reported by Ward's. Specifically, we define a model-year plus trim's dealer cost as the average dealer cost for the model-year vehicle with which it is associated plus the deviation of the model-year variant specific MSRP from the average MSRP across all variants of that model-year. 
	 
	\subsection{``Arbitrary'' Initial Conditions}
	\label{ECSUBSEC:InitialConditions}
	
	Our ``arbitrary'' initial conditions used in Section \ref{SUBSEC:Sensitivity} were formally defined as follows. For the \citeauthor{Boyd80} model initial conditions are drawn uniformly from $[ \min_{j \in \N(J)} c_j , \max_{j \in \N(J)} c_j ]^J$. For the \citeauthor{Berry95} model, the finite reservation price (income) makes choosing arbitrary initial conditions more difficult. We draw initial conditions uniformly from $[0,19000]^J$, where the $70\ith$ percentile of income is approximately $19,000$ 1983 USD. Using this upper limit ensures that, loosely speaking, the upper 30 \% of the sampled population can buy {\em any} vehicle at the initial prices, and does {\em not} preclude the existence of individuals in the sampled population that have an income too low to buy any of the vehicles at their initial prices. 
	 
	\subsection{Additional Results}
	
	\subsubsection{Cost Trials}
	
	Table \ref{TAB:CostCompDetailed} provides detailed results regarding our trials starting at unit costs. 
	
	\begin{table}
		\TABLE
		{Results of price equilibrium computations starting at unit costs under both demand models for ten $1,000$-sample sets. $n$: iterations to termination (maximum is 75); $t$: CPU time (in seconds); ``FO'': First-order conditions satisfied (``S'') or failed (``F''); ``SO'': Second-order conditions satisfied (``S'') or failed (``F''); $\abs{ \vec{p}_* - \vec{p}_*^{\text{FPI}}}$: absolute deviation from equilibrium prices computed by $\bsym{\zeta}$-FPI (in 1980 and 1983 USD). \label{TAB:CostCompDetailed}}
		{\begin{tabular}{cccccccccccccccccccccccccccccccccccccc}
			\\
			\multicolumn{7}{c}{\cite{Boyd80}} && \multicolumn{7}{c}{\cite{Berry95}} \\ \cline{1-7} \cline{9-15} \\
			\\
			\multicolumn{7}{c}{$\bsym{\eta}$-NM} && \multicolumn{7}{c}{$\bsym{\eta}$-NM} \\ \cline{1-7} \cline{9-15}
			&&&& \multicolumn{3}{c}{$\abs{ \vec{p}_* - \vec{p}_*^{\text{FPI}} }$} &&&&&&& \multicolumn{3}{c}{$\abs{ \vec{p}_* - \vec{p}_*^{\text{FPI}} }$} \\ \cline{5-7} \cline{13-15}
		$n$	&	$t$ 		&	FO	&	SO	& min 		& median 		& max 		&	&	$n$	&	$t$		&	FO	&	SO	&	min		&	median	&	max	\\ \cline{1-7} \cline{9-15}
		8	&	77.32	&	S	&	S	&	1.30E-06	&	1.84E-03	&	5.68E+00	&	&	5	&	52.64	&	S	&	S	&	8.97E-05	&	4.20E-02	&	1.16E+02	\\
		75	&	530.51	&	F	&	F	&	6.88E-02	&	1.84E+02	&	6.27E+04	&	&	7	&	65.56	&	S	&	S	&	8.71E-04	&	3.13E-02	&	1.44E+01	\\
		8	&	75.62	&	S	&	S	&	8.15E-05	&	8.01E-03	&	7.61E+00	&	&	5	&	50.67	&	S	&	S	&	1.90E-07	&	1.12E-04	&	1.78E-02	\\
		75	&	508.77	&	F	&	F	&	7.06E-03	&	8.56E+01	&	7.28E+03	&	&	5	&	52.2		&	S	&	S	&	3.29E-06	&	4.13E-03	&	5.47E+00	\\
		13	&	113.66	&	S	&	S	&	1.16E-04	&	8.11E-03	&	7.58E+00	&	&	5	&	52.84	&	S	&	S	&	2.80E-06	&	8.54E-04	&	2.26E+00	\\
		14	&	122.84	&	S	&	S	&	1.95E-06	&	8.54E-03	&	9.80E+00	&	&	5	&	50.47	&	S	&	S	&	6.81E-07	&	5.01E-04	&	3.59E-03	\\
		9	&	86.64	&	S	&	S	&	1.31E-04	&	1.06E-02	&	1.29E+01	&	&	5	&	50.52	&	S	&	S	&	5.36E-08	&	5.27E-04	&	3.88E-03	\\
		7	&	70.62	&	S	&	S	&	5.32E-04	&	1.37E-02	&	1.33E+01	&	&	7	&	63.38	&	S	&	S	&	9.86E-08	&	7.77E-05	&	1.27E-03	\\
		75	&	556.99	&	F	&	F	&	8.66E-02	&	2.77E+01	&	4.52E+04	&	&	5	&	50.8	&	S	&	S	&	8.56E-06	&	1.14E-04	&	1.62E-03	\\
		11	&	100.06	&	S	&	S	&	1.57E-05	&	2.10E-03	&	4.29E-01	&	&	8	&	69.5	&	S	&	S	&	2.07E-06	&	5.85E-04	&	1.64E-02	\\\cline{1-7} \cline{9-15}
		8	&	70.62	&	min	&		&		&		&		&	&	6	&	50.47	&	min	&		&		&		&		\\
		10	&	86.64	&	med	&		&		&		&		&	&	6	&	52.42	&	med	&		&		&		&		\\
		15	&	122.84	&	max	&		&		&		&		&	&	9	&	69.5	&	max	&		&		&		&		\\ \cline{1-7} \cline{9-15}
			\\
			\multicolumn{7}{c}{$\bsym{\zeta}$-NM} && \multicolumn{7}{c}{$\bsym{\zeta}$-NM} \\ \cline{1-7} \cline{9-15}
			&&&& \multicolumn{3}{c}{$\abs{ \vec{p}_* - \vec{p}_*^{\text{FPI}} }$} &&&&&&& \multicolumn{3}{c}{$\abs{ \vec{p}_* - \vec{p}_*^{\text{FPI}} }$} \\ \cline{5-7} \cline{13-15}
		$n$	&	$t$ 	&	FO	&	SO	& min & median & max &	&	$n$	&	$t$	&	FO	&	SO	&	min	&	median	&	max	\\ \cline{1-7} \cline{9-15}
		17	&	125.56	&	S	&	S	&	2.59E-06	&	1.84E-03	&	5.63E+00	&	&	7	&	64.21	&	S	&	S	&	4.21E-05	&	4.39E-02	&	1.22E+02	\\
		9	&	80.35	&	S	&	S	&	4.99E-05	&	1.06E-02	&	2.22E+01	&	&	8	&	70.11	&	S	&	S	&	1.03E-03	&	2.97E-02	&	1.27E+01	\\
		12	&	108.67	&	S	&	S	&	6.47E-05	&	8.01E-03	&	7.61E+00	&	&	29	&	257.25	&	F	&	F	&	3.62E-06	&	5.19E-02	&	2.48E+00	\\
		75	&	507.52	&	F	&	F	&	9.78E-02	&	6.79E+01	&	5.62E+03	&	&	8	&	69.67	&	S	&	S	&	2.36E-04	&	6.41E-03	&	9.58E+00	\\
		75	&	501.52	&	F	&	F	&	7.81E-02	&	2.58E+02	&	1.58E+04	&	&	7	&	65.53	&	S	&	S	&	3.48E-07	&	1.22E-03	&	5.20E-01	\\
		14	&	116.82	&	S	&	S	&	8.12E-06	&	8.55E-03	&	9.80E+00	&	&	10	&	90.16	&	S	&	S	&	7.07E-06	&	6.83E-04	&	3.87E-03	\\
		14	&	119.12	&	S	&	S	&	4.45E-05	&	1.07E-02	&	1.29E+01	&	&	9	&	75.2		&	S	&	S	&	2.27E-07	&	5.92E-04	&	4.42E-03	\\
		19	&	147.41	&	S	&	S	&	3.31E-05	&	1.35E-02	&	1.33E+01	&	&	8	&	72.62	&	S	&	S	&	1.88E-07	&	6.27E-04	&	5.04E-03	\\
		75	&	556.26	&	F	&	F	&	2.32E-03	&	2.43E+01	&	4.51E+04	&	&	8	&	74.91	&	S	&	S	&	1.55E-07	&	4.41E-04	&	3.54E-03	\\
		75	&	508.17	&	F	&	F	&	2.37E-01	&	1.03E+02	&	6.60E+04	&	&	8	&	72.88	&	S	&	S	&	9.80E-06	&	7.09E-04	&	6.63E-03	\\	\\ \cline{1-7} \cline{9-15}
		10	&	80.35	&	min	&		&		&		&		&	&	8	&	64.21	&	min	&		&		&		&		\\
		15	&	117.97	&	med	&		&		&		&		&	&	9	&	72.62	&	med	&		&		&		&		\\
		20	&	147.41	&	max	&		&		&		&		&	&	11	&	90.16	&	max	&		&		&		&		\\ \cline{1-7} \cline{9-15}
		\\
			\multicolumn{4}{c}{$\bsym{\zeta}$-FPI} &&&&& \multicolumn{4}{c}{$\bsym{\zeta}$-FPI} \\ \cline{1-4} \cline{9-12}
		$n$	&	$t$	&	FO	&	SO	&		&		&		&	&	$n$	&	$t$	&	FO	&	SO	&		&		&		\\ \cline{1-4} \cline{9-12}
		24	&	18.07	&	S	&	S	&		&		&		&	&	19	&	24.35	&	S	&	S	&		&		&		\\
		70	&	52.58	&	S	&	S	&		&		&		&	&	18	&	22.58	&	S	&	S	&		&		&		\\
		36	&	27.58	&	S	&	S	&		&		&		&	&	22	&	27.47	&	S	&	S	&		&		&		\\
		29	&	22.02	&	S	&	S	&		&		&		&	&	19	&	23.83	&	S	&	S	&		&		&		\\
		53	&	40.26	&	S	&	S	&		&		&		&	&	19	&	23.9	&	S	&	S	&		&		&		\\
		41	&	31.29	&	S	&	S	&		&		&		&	&	19	&	23.7	&	S	&	S	&		&		&		\\
		39	&	29.74	&	S	&	S	&		&		&		&	&	20	&	24.98	&	S	&	S	&		&		&		\\
		38	&	28.93	&	S	&	S	&		&		&		&	&	23	&	28.62	&	S	&	S	&		&		&		\\
		44	&	33.62	&	S	&	S	&		&		&		&	&	22	&	27.39	&	S	&	S	&		&		&		\\
		23	&	17.37	&	S	&	S	&		&		&		&	&	19	&	23.56	&	S	&	S	&		&		&		\\ \cline{1-4} \cline{9-12}
		23	&	17.37	&	min	&		&		&		&		&	&	18	&	22.58	&	min	&		&		&		&		\\
		38.5	&	29.335	&	med	&		&		&		&		&	&	19	&	24.125	&	med	&		&		&		&		\\
		70	&	52.58	&	max	&		&		&		&		&	&	23	&	28.62	&	max	&		&		&		&		\\ \cline{1-4} \cline{9-12}
			\\
			\\ \cline{1-15}\cline{1-15}
		\end{tabular}}
		{}
	\end{table}

==> simpleexample.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Simple Example}
\label{ECSEC:SimpleExample}

In this section we elaborate on Example \ref{EX:SimpleExample}. Recall that $\vec{F} : \R^N \to \R^N$ is given by $\vec{F}(\vec{x}) = \vec{x}/(1 + \norm{\vec{x}}_2^2)$, has a unique finite zero at $\vec{0}$, and vanishes as $\norm{\vec{x}}_2 \to \infty$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Pure Newton}

We first note that
\begin{equation*}
	(D\vec{F})(\vec{x})
		= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right) \left[ \vec{I} - \left( \frac{2}{1+\norm{\vec{x}}_2^2} \right) \vec{x}\vec{x}^\top \right]. 
\end{equation*}
$(D\vec{F})(\vec{x})$ is nonsingular only if $\norm{\vec{x}}_2 \neq 1$. 

By the Sherman-Morrison-Woodbury formula \citep{Ortega70, Dennis96}, 
\begin{equation*}
	(D\vec{F})(\vec{x})\inv
		= \left( 1+\norm{\vec{x}}_2^2 \right) \left[ \vec{I} + \left( \frac{2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}\vec{x}^\top \right]
\end{equation*}
so long as $\norm{\vec{x}}_2 \neq 1$. Thus the Newton step, $\vec{s}^N$, is
\begin{equation*}
	\vec{s}^N
		= - (D\vec{F})(\vec{x})\inv\vec{F}(\vec{x})
%		= - \left[ \vec{I} + \left( \frac{2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}\vec{x}^\top \right] \vec{x}
		= - \left( 1 + \frac{2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}
%		= - \left( \frac{1-\norm{\vec{x}}_2^2+2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}
		= - \left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}
\end{equation*}
The Newton point $\vec{x} + \vec{s}^N$ is thus given by
\begin{equation*}
	\vec{x} + \vec{s}^N
		= - \left( \frac{2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}. 
\end{equation*}

We consider convergence of the pure Newton iteration to $\vec{0}$. Note that
\begin{align*}
	\norm{ \vec{x} + \vec{s}^N - \vec{0} }_2
		= \left( \frac{ 2\norm{\vec{x}}_2^2 }{\abs{ 1-\norm{\vec{x}}_2^2} } \right) \norm{ \vec{x} - \vec{0} }_2
\end{align*}
and thus the Newton step reduces the 2-norm error in $\vec{x}$ only if
\begin{align*}
	2\norm{\vec{x}}_2^2 < \abs{ 1-\norm{\vec{x}}_2^2}. 
\end{align*}
This inequality is satisfied only if $\norm{\vec{x}}_2 < 1/\sqrt{3}$ as can be easily checked. Thus
\begin{align*}
	\norm{ \vec{x} + \vec{s}^N - \vec{0} }_2
		\; \left\{ \begin{aligned}
			< \norm{ \vec{x} - \vec{0} }_2 &\quad\text{if } \norm{\vec{x}}_2 < 1/\sqrt{3} \\
			= \norm{ \vec{x} - \vec{0} }_2 &\quad\text{if } \norm{\vec{x}}_2 = 1/\sqrt{3} \\
			> \norm{ \vec{x} - \vec{0} }_2 &\quad\text{if } \norm{\vec{x}}_2 > 1/\sqrt{3}, \norm{\vec{x}}_2 \neq 1
		\end{aligned} \right .
\end{align*}
Furthermore
\begin{equation*}
	\abs{ x_n + s_n^N } = \left( \frac{ 2\norm{\vec{x}}_2^2 }{\abs{ 1-\norm{\vec{x}}_2^2} } \right) \abs{ x_k }
\end{equation*}
and thus the Newton step increases the absolute value of {\em every} nonzero component of $\vec{x}$ when $\norm{\vec{x}}_2 > 1/\sqrt{3}$ ($\norm{\vec{x}}_2 \neq 1$). When $\norm{\vec{x}}_2 \in (1/\sqrt{3},1)$, the Newton steps also enforce an alternation in the signs of the components of $\vec{x}$. If $\norm{\vec{x}}_2 = 1/\sqrt{3}$ the Newton point is $-\vec{x}$. 

The Newton iterates diverge if $\norm{\vec{x}^{(0)}}_2 > 1/\sqrt{3}$ simply because $\norm{\vec{s}^N(\vec{x}^{(n)})}_2$ cannot vanish; indeed, if $\norm{\vec{x}^{(n)}}_2 \to \gamma \notin \{ 0,1 \} $ then 
\begin{equation*}
	\norm{\vec{x}^{(n+1)} - \vec{x}^{(n)} }_2 
		= \norm{\vec{s}^N(\vec{x}^{(n)})}_2 
		\to \left( \frac{1 + \gamma^2}{\abs{1 - \gamma^2}} \right) \gamma
		\neq 0. 
\end{equation*}

Note also that
\begin{equation*}
	1 = \norm{ \vec{x} + \vec{s}^N }_2
		= \frac{2\norm{\vec{x}}_2^3}{\abs{1-\norm{\vec{x}}_2^2}}
\end{equation*}
requires $\norm{\vec{x}}_2 \in (1/\sqrt{3},1)$, because otherwise $\norm{ \vec{x} + \vec{s}^N }_2 \leq \norm{ \vec{x} }_2 \leq 1/\sqrt{3}$ or $\norm{ \vec{x} + \vec{s}^N }_2 > \norm{ \vec{x} }_2 > 1$. Now $\psi(a) = 2a^3/(1-a^2)$ is an increasing function on $[1/\sqrt{3},1)$ with $\psi(1/\sqrt{3}) = 1/\sqrt{3}$ and $\psi(a) \to \infty$ as $a \uparrow 1$. Thus for {\em any} $\gamma \in (1/\sqrt{3},1]$ there is a unique $\psi^{-1}(\gamma) \in (1/\sqrt{3},1)$ such that $\psi(\psi^{-1}(\gamma)) = \gamma$. Define a sequence of radii $\{ r_n \}_{n=0}^\infty$ by $r_0 = 1$ and $r_n = \psi^{-1}(r_{n-1}) = \psi^{-n}(1)$, $n \geq 1$, where $\psi^{-n}$ is the $n\ith$ is the inverse map $\psi^{-1}$ iterated $n$ times. Some iterate in the Newton sequence falls on the unit sphere if, and only if, $\norm{ \vec{x}^{(0)} }_2 = r_n$ for some $n \in \{0,1,2,\dotsc,\}$. 

\subsection{Line Search}

Line search takes the update $\vec{x} + \lambda \vec{s}^N/\norm{\vec{s}^N}_2$ for some step length $\lambda$. We make two observations based on the formula 
\begin{equation*}
	\frac{\vec{s}^N}{\norm{\vec{s}^N}_2}
		= - \mathrm{sign}\left\{ \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right\} \left( \frac{\vec{x}}{\norm{\vec{x}}_2} \right). 
\end{equation*}
First, {\em there is always an exact line search step to} $\vec{0}$. Specifically, if 
\begin{align*}
%	\vec{0} 
%		&= \vec{x} + \lambda \left( \frac{\vec{s}^N}{\norm{\vec{s}^N}_2} \right) \\
%		&= \vec{x} - \lambda \; \mathrm{sign}\left\{ \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right\} \left( \frac{\vec{x}}{\norm{\vec{x}}_2} \right) \\
%	1 &= \mathrm{sign}\left\{ \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right\} \left( \frac{\lambda}{\norm{\vec{x}}_2} \right) \\
	\lambda &= \mathrm{sign}\left\{ \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right\} \norm{\vec{x}}_2
\end{align*}
then $\vec{x} + \lambda \vec{s}^N/\norm{\vec{s}^N}_2 = \vec{0}$. Second, {\em if $\norm{\vec{x}}_2 > 1$ then any line search step with positive step length increases the distance to} $\vec{0}$. This is because $\vec{x} + \lambda \vec{s}^N / \norm{\vec{s}^N}_2 = (1 + \lambda\norm{\vec{x}}_2\inv) \vec{x}$. If $\norm{\vec{x}}_2 \in [1/\sqrt{3},1)$ the line search may enforce convergence that did not occur with the pure Newton method. 

Unfortunately most step length finding methods use only positive step lengths (generally for good reason). For example, a simple backtracking line search sets $\lambda = 2^{-m_*} > 0$ where
\begin{equation*}
	m_* = \inf \left\{ \norm{ \vec{F}(\vec{x}+2^{-m}\vec{s}^N) }_2 < ( 1 - \alpha 2^{-m} ) \norm{ \vec{F}(\vec{x}) }_2 \right\}. 
\end{equation*}
Another popular choice forms a quadratic model of $\norm{\vec{F}(\vec{x}+\lambda \vec{s}^N)}_2$ and computes its minimizer, ``safeguarding'' the steplength to be some positive bounded fraction of the previous steplength. This method also generally computes only positive steplengths, and thus will diverge for $\norm{\vec{x}}_2 > 1$. 

%Note that
%\begin{equation*}
%	\norm{ \vec{F}(\vec{x}) }_2 = \frac{\norm{\vec{x}}_2}{1+\norm{\vec{x}}_2^2}
%\end{equation*}
%\begin{align*}
%	\vec{x} + 2^{-m}\vec{s}^N
%%		&= \vec{x} - 2^{-m} \left( 1 + \frac{2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
%%		&= \left( 1 - 2^{-m} - 2^{-m} \frac{2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
%%		&= 2^{-m} \left( 2^m - 1 - \frac{2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
%%		&= 2^{-m} \left( \frac{( 2^m - 1)( 1 - \norm{\vec{x}}_2^2) - 2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
%%		&= 2^{-m} \left( \frac{(2^m-1) - (2^m-1)\norm{\vec{x}}_2^2 - 2\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
%		&= 2^{-m} \left( \frac{(2^m-1) - (2^m+1)\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x}
%\end{align*}
%Thus
%\begin{align*}
%	\norm{ \vec{x} + 2^{-m}\vec{s}^N }_2
%		&= 2^{-m} \abs{ \frac{(2^m-1) - (2^m+1)\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} } \norm{ \vec{x} }_2 \\
%		&= A(m) \norm{\vec{x}}_2
%\end{align*}
%where
%\begin{align*}
%	A(m) = 2^{-m} \abs{ \frac{(2^m-1) - (2^m+1)\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} }
%\end{align*}
%and
%\begin{align*}
%	\norm{ \vec{F}(\vec{x} + 2^{-m}\vec{s}^N) }_2 
%		&= \frac{ A(m) \norm{\vec{x}}_2 }{ 2^m + A(m)^2 \norm{\vec{x}}_2^2 }
%\end{align*}
%Note that
%\begin{align*}
%	\norm{ \vec{F}(\vec{x} + 2^{-m}\vec{s}^N) }_2 + \alpha 2^{-m} \norm{ \vec{F}(\vec{x}) }_2
%		&= \frac{ A \norm{\vec{x}}_2 }{ 1 + A^2 \norm{\vec{x}}_2^2 } + \alpha 2^{-m} \frac{\norm{\vec{x}}_2}{1+\norm{\vec{x}}_2^2} \\
%		&= \left( \frac{ \norm{\vec{x}}_2 }{1+\norm{\vec{x}}_2^2} \right) \left[ \frac{ A( 1 + \norm{\vec{x}}_2^2 ) }{ 1 + A^2 \norm{\vec{x}}_2^2 } + \alpha 2^{-m} \right] \\
%		&= \norm{ \vec{F}(\vec{x}) }_2 \left[ \frac{ A( 1 + \norm{\vec{x}}_2^2 ) }{ 1 + A^2 \norm{\vec{x}}_2^2 } + \alpha 2^{-m} \right]
%\end{align*}
%Thus
%\begin{align*}
%	\norm{ \vec{F}(\vec{x} + 2^{-m}\vec{s}^N) }_2 + \alpha 2^{-m} \norm{ \vec{F}(\vec{x}) }_2 < \norm{ \vec{F}(\vec{x}) }_2
%\end{align*}
%only if
%\begin{align*}
%	\frac{ A( 1 + \norm{\vec{x}}_2^2 ) }{ 1 + A^2 \norm{\vec{x}}_2^2 } + \alpha 2^{-m} &< 1 \\
%	A(m)( 1 + \norm{\vec{x}}_2^2 ) &< ( 1 - \alpha 2^{-m} ) ( 1 + A(m)^2 \norm{\vec{x}}_2^2 ) \\
%	A(m)( 1 + \norm{\vec{x}}_2^2 ) &< ( 1 - \alpha 2^{-m} ) \norm{\vec{x}}_2^2 A(m)^2 + ( 1 - \alpha 2^{-m} ) \\
%	1 + \norm{\vec{x}}_2^2 &< ( 1 - \alpha 2^{-m} ) \norm{\vec{x}}_2^2 A(m) + ( 1 - \alpha 2^{-m} ) A(m)\inv \\
%	\frac{ 1 + \norm{\vec{x}}_2^2 }{ 1 - \alpha 2^{-m} } 
%		&< \norm{\vec{x}}_2^2 2^{-m} \abs{ \frac{(2^m-1) - (2^m+1)\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} }
%			 + 2^m \abs{ \frac{1-\norm{\vec{x}}_2^2}{(2^m-1) - (2^m+1)\norm{\vec{x}}_2^2} } \\
%\end{align*}

\subsection{Trust Region Methods}

Trust region methods try to minimize $\varphi(\vec{x}) = (1/2)\norm{\vec{F}(\vec{x}+\vec{s})}_2$ subject to the constraint that $\norm{\vec{s}}_2 \leq \delta$. This is itself a difficult nonlinear optimization problem, and thus practical trust region methods are based on minimizing the following quadratic local model of $\varphi$ instead:
\begin{equation*}
	m_\vec{x}(\vec{s}) 
		= \left( \frac{1}{2} \right) \norm{\vec{F}(\vec{x})}_2^2
			+ \vec{F}(\vec{x})^\top(D\vec{F})(\vec{x})\vec{s}
			+ \left( \frac{1}{2} \right) \vec{s}^\top (D\vec{F})(\vec{x})^\top (D\vec{F})(\vec{x})\vec{s}
\end{equation*}

\subsubsection{Levenburg-Marquardt Method or Hookstep}

Minimizing this quadratic model subject to the constraint $\norm{\vec{s}}_2 \leq \delta$ is conceptually straightforward: either (i) $\norm{ \vec{s}^N }_2 \leq \delta$ and then $\vec{s}^L = \vec{s}^N$, or (ii) $\norm{ \vec{s}^N }_2 > \delta$ and we take $\vec{s}^L = \vec{s}(\lambda_*)$ where $\vec{s}(\lambda)$ solves
\begin{equation*}
	\Big( (D\vec{F})(\vec{x})^\top (D\vec{F})(\vec{x}) + \lambda \vec{I} \Big) \vec{s}(\lambda)
		= - (D\vec{F})(\vec{x})^\top\vec{F}(\vec{x})
\end{equation*}
and $\lambda_* > 0$ is the unique solution to $\norm{ \vec{s}(\lambda) }_2 = \delta$. 

Now
\begin{equation*}
	(D\vec{F})(\vec{x})^\top\vec{F}(\vec{x})
		= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x}
\end{equation*}
and
\begin{equation*}
	(D\vec{F})(\vec{x})^\top(D\vec{F})(\vec{x})
		= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2
			\left[ \vec{I} - \left( \frac{2}{1+\norm{\vec{x}}_2^2} \right)^2 \vec{x}\vec{x}^\top \right]
\end{equation*}
One can verify that the Newton step is recovered from the $\lambda = 0$ case,
\begin{equation*}
	(D\vec{F})(\vec{x})^\top(D\vec{F})(\vec{x})\vec{s}(0) = - (D\vec{F})(\vec{x})^\top\vec{F}(\vec{x}),
\end{equation*}
also called the ``normal equation.''

In general the LM system is
\begin{align*}
	\left\{ 
		\left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2
			\left[ \vec{I} - \left( \frac{2}{1+\norm{\vec{x}}_2^2} \right)^2 \vec{x}\vec{x}^\top \right]
			+ \lambda \vec{I}
		\right\} \vec{s}(\lambda)
		&= - \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
	\left[ \big( 1 +  \lambda(1+\norm{\vec{x}}_2^2)^2 \big) \vec{I} - \left( \frac{2}{1+\norm{\vec{x}}_2^2} \right)^2 \vec{x}\vec{x}^\top \right]
			\vec{s}(\lambda)
		&= - \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
\end{align*}
Define $\Lambda = 1 + \lambda( 1 + \norm{\vec{x}}_2^2 )^2$ and $A = 2/(1+\norm{\vec{x}}_2^2)$. Then 
\begin{align*}
	\left[ \Lambda \vec{I} - A^2 \vec{x}\vec{x}^\top \right]
			\vec{s}(\lambda)
		&= - \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
	\left[ \vec{I} - \left( \frac{A^2}{\Lambda} \right) \vec{x}\vec{x}^\top \right]
			\vec{s}(\lambda)
		&= - \left( \frac{1}{\Lambda} \right) \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
	\vec{s}(\lambda)
		&= - \left( \frac{1}{\Lambda} \right) \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) 
				\left[ \vec{I} + \left( \frac{A^2}{\Lambda - A^2\norm{\vec{x}}_2^2} \right) \vec{x}\vec{x}^\top \right]
			\vec{x} \\
		&= - \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) 
				\left( \frac{1}{\Lambda - A^2\norm{\vec{x}}_2^2} \right)
			\vec{x}
\end{align*}
If $\norm{\vec{x}}_2 > 1$ and $\Lambda > A^2\norm{\vec{x}}_2^2$, then $\vec{s}(\lambda)$ increases the distance to the origin. 

Now $\Lambda > A^2\norm{\vec{x}}_2^2$ if, and only if, 
\begin{align*}
%	1 + \lambda( 1 + \norm{\vec{x}}_2^2 )^2 &> \frac{2}{1+\norm{\vec{x}}_2^2} \\
%	(1+\norm{\vec{x}}_2^2) + \lambda( 1 + \norm{\vec{x}}_2^2 )^3 &> 2 \\
%	\lambda( 1 + \norm{\vec{x}}_2^2 )^3 &> 1  - \norm{\vec{x}}_2^2  \\
%	\lambda &> \frac{ 1  - \norm{\vec{x}}_2^2 }{( 1 + \norm{\vec{x}}_2^2 )^3} \\
	\lambda &> \left( \frac{ 1  }{1 + \norm{\vec{x}}_2^2} \right)^2
					\left( \frac{ 1  - \norm{\vec{x}}_2^2 }{1 + \norm{\vec{x}}_2^2} \right)
\end{align*}
Note that if $\norm{\vec{x}}_2 > 1$, then this inequality is trivially satisfied for all $\lambda \geq 0$. In other words, the hookstep also increases the length of $\vec{x}$, and thus does not enforce global convergence to $\vec{0}$ for $\norm{\vec{x}^{(0)}}_2 > 1$. 

\subsubsection{Powell's Hybrid Method or Dogleg Step}

Powell's Hybrid method or the Dogleg step $\vec{s}^D$ is the Newton step if $\norm{ \vec{s}^N }_2 \leq \delta$, otherwise is the unique step of 2-norm $\delta$ on the piecewise linear path from $\vec{0}$ to the Cauchy step $\vec{s}^C$ (defined below) and then to the Newton step. This does not alleviate the poor global convergence behavior because {\em the Cauchy point and the Newton point coincide}. Thus the dogleg step is simply a scaled Newton step: $\vec{s}^D = \min\{ \norm{\vec{s}^N}_2,\delta\} \vec{s}^N / \norm{\vec{s}^N}_2$. If $\norm{\vec{x}}_2^2 > 1$, this step points increases all components of $\vec{x}$ and, regardless of $\delta$, $\norm{\vec{x}+\vec{s}^D}_2^2 > 1$ again. If $\norm{\vec{x}}_2^2 < 1$, this step points in the right direction and the scaling could effectively enforce convergence to $\vec{0}$. In the remainder of this section we prove our claim that the Cauchy point and the Newton point coincide. 

We first compute the steepest descent direction for $\varphi(\vec{x}) = (1/2)\norm{\vec{F}(\vec{x})}_2$:
\begin{equation*}
	\vec{d} = (D\vec{F})(\vec{x})^\top\vec{F}(\vec{x})
		= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x}
\end{equation*}
Note that the steepest descent steps, like the Newton step, also just re-scale $\vec{x}$. The Cauchy step $\vec{s}^C$ is the minimizer of $m_\vec{x}(\vec{s}) $ in the steepest descent direction. Since
\begin{equation*}
	m_\vec{x}(\alpha\vec{d}) 
		= \left( \frac{1}{2} \right) \norm{\vec{F}(\vec{x})}_2^2
			+ \alpha \norm{ \vec{d} }_2^2
			+ \left( \frac{\alpha^2}{2} \right) \norm{ (D\vec{F})(\vec{x})\vec{d} }_2^2
\end{equation*}
we must have
\begin{equation*}
	\alpha = - \frac{ \norm{ \vec{d} }_2^2 }{ \norm{ (D\vec{F})(\vec{x})\vec{d} }_2^2 }. 
\end{equation*}
However note that
\begin{align*}
	(D\vec{F})(\vec{x})\vec{d} 
		&= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) 
				(D\vec{F})(\vec{x})\vec{x} \\
		&= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^3 \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) 
				\left( 1 - \frac{2\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
		&= \left( \frac{1}{1+\norm{\vec{x}}_2^2} \right) \left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{d}
\end{align*}
so that
\begin{equation*}
	\alpha = - \left( 1+\norm{\vec{x}}_2^2 \right)^2 \left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right)^2
\end{equation*}
and
\begin{align*}
	\vec{s}^C 
		= \alpha\vec{d} 
		&= - \left( 1+\norm{\vec{x}}_2^2 \right)^2 \left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right)^2
				\left( \frac{1}{1+\norm{\vec{x}}_2^2} \right)^2\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
		&= - \left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right)^2
				\left( \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right) \vec{x} \\
		&= - \mathrm{sign}\left\{ \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right\}
				\abs{ \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} } \vec{x} \\
		&= - \mathrm{sign}\left\{ \frac{1-\norm{\vec{x}}_2^2}{1+\norm{\vec{x}}_2^2} \right\}^2
				\left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
		&= - \left( \frac{1+\norm{\vec{x}}_2^2}{1-\norm{\vec{x}}_2^2} \right) \vec{x} \\
		&= \vec{s}^N
\end{align*}
That is, the Cauchy step {\em is} the Newton step, and thus the Cauchy and Newton points coincide. The dogleg step is thus a line search method, and cannot enforce global convergence to $\vec{0}$ for $\norm{ \vec{x}^{(0)} }_2 > 1$. 
